Efficient Latency-Aware CNN Depth Compression via Two-Stage Dynamic Programming

Recent works on neural network pruning advocate that reducing the depth of the network is more effective in reducing run-time memory usage and accelerating inference latency than reducing the width of the network through channel pruning. In this regard, some recent works propose depth compression algorithms that merge convolution layers. However, the existing algorithms have a constricted search space and rely on human-engineered heuristics. In this paper, we propose a novel depth compression algorithm which targets general convolution operations. We propose a subset selection problem that replaces inefficient activation layers with identity functions and optimally merges consecutive convolution operations into shallow equivalent convolution operations for efficient end-to-end inference latency. Since the proposed subset selection problem is NP-hard, we formulate a surrogate optimization problem that can be solved exactly via two-stage dynamic programming within a few seconds. We evaluate our methods and baselines by TensorRT for a fair inference latency comparison. Our method outperforms the baseline method with higher accuracy and faster inference speed in MobileNetV2 on the ImageNet dataset. Specifically, we achieve $1.41\times$ speed-up with $0.11$\%p accuracy gain in MobileNetV2-1.0 on the ImageNet.

==> equation/accsurrogate.tex <==
\begin{align*}
\sum_{i=0}^{|A|} I[a_i, a_{i+1}]
\end{align*}


==> equation/activeindexset.tex <==
\begin{align}
    \label{eq:activeindexset}
    A \coloneqq \left\{ l\in [L-1] \mid \sigma_l \neq \text{id}_X \right\}.
\end{align}



==> equation/dprecurmain.tex <==
\begin{align}
    \label{eq:dprecur}
    k&= \underset{k' \subseteq [l-1]}{\mathrm{argmax}} ~ I(A[k', t- T_\text{opt}[k',l]] \cup \{k'\},0, l)\nonumber\\
    A[l, t] &= A[k, t- T_\text{opt}[k,l]] \cup \{k\}\nonumber\\
    S[l, t] &= S[k, t- T_\text{opt}[k,l]] \cup \{k\}\cup S_\text{opt}[k,l] 
\end{align}


==> equation/dptable2.tex <==
\begin{subequations}
\begin{align}
    D[l,t] \coloneqq &\underset{A,S \subseteq [l-1]}{\mathrm{max}} \;\; I(A,0,l)\label{eq:dptable1}\\
    &\mathrm{subject\ to\ } \;\; 
    T(S,0,l)< t, \nonumber\\
    A[l,t], S[l,t] \coloneqq &\underset{A,S \subseteq [l-1]}{\mathrm{argmax}} \;\; I(A,0,l) \label{eq:dptable2}\\
    &\mathrm{subject\ to\ } \;\; 
    T(S,0,l)< t, \nonumber
\end{align}
\label{eq:dptable}
\end{subequations}


==> equation/latency2.tex <==
\begin{align}
\label{eq:latency2}
    T(S) \triangleq \sum_{i=1}^{|S|+1} T[s_{i-1},s_i]<T_0.
\end{align}


==> equation/networkinference.tex <==
\begin{align*}
    x^{(0)} &= x\\
    x^{(l)} &= \sigma_l (f_{\theta_l}(x^{(l-1)}))\quad \forall ~l\in \{1,\ldots, L\},
\end{align*}


==> equation/opt2.tex <==
\footnotesize
\begin{align}
\label{eq:opt2}
    &\underset{A,S \subseteq [L-1]}{\mathrm{maximize}} ~~\underset{\theta^*}{\mathrm{max}}\;\mathrm{Acc}\left( 
    \BigO_{l=1}^L \left( \mathds{1}_A(l)\sigma_l + \left(1-\mathds{1}_A(l)\right) \mathrm{id} \right) \circ f_{\theta_l} \right)\nonumber\\
    &\mathrm{subject\ to\ }~~ T(S)<T_0, ~A\subseteq S.
\end{align}
\normalsize


==> equation/timedpmain.tex <==
\begin{align*}
    T_{\text{opt}}[k,l] &\coloneqq \min_{S \subseteq \{ k\!+\!1,\ldots,l\!-\!1\}} T(S,k,l)\\
    S_{\text{opt}}[k,l] &\coloneqq \underset{S \subseteq \{ k\!+\!1,\ldots,l\!-\!1\}}{\mathrm{argmin}} T(S,k,l).
\end{align*}

==> fig/convfilter.tex <==
\begin{figure}

\def\xshift{113}
\resizebox{\columnwidth}{!}{
\centering
\pgfdeclarelayer{ka}\pgfdeclarelayer{kb}\pgfdeclarelayer{kc}
\pgfsetlayers{ka,kb,kc}  
\begin{tikzpicture}[decoration={brace}][scale=1,every node/.style={minimum size=1cm},on grid]
\begin{pgfonlayer}{ka}
       \begin{scope}[  
        xshift=0,
             every node/.append style={}]

        \foreach \x in {0,1,2} {
            \foreach \y in {0,1,2} {
                \draw[blue!100,thick] (\x,\y) rectangle (\x+1,\y+1);
                \filldraw[cyan!30, opacity=0.7] (\x,\y) rectangle (\x+1,\y+1);
                \node at (\x+0.5,\y+0.5) {1};
        }
    }
    \draw[black!100,thick] (0,0) rectangle (3,3);
    \node at (3.5, 1.5) {\Huge$\ast$};
    \node at (1.5, -0.5) {\Large$K_1$};
    \end{scope}
\end{pgfonlayer}
\begin{pgfonlayer}{kb}
       \begin{scope}[  
        xshift=\xshift,
             every node/.append style={}]

        \foreach \x in {0,1,2} {
            \foreach \y in {0,1,2} {
                \draw[blue!100,thick] (\x,\y) rectangle (\x+1,\y+1);
                \filldraw[magenta!30, opacity=0.7] (\x,\y) rectangle (\x+1,\y+1);
                \node at (\x+0.5,\y+0.5) {1};
        }
                \draw[black!100,thick] (0,0) rectangle (3,3);
    }
    \node at (3.5, 1.5) {\Huge$=$};
    \node at (1.5, -0.5) {\Large$K_2$};
    \end{scope}
\end{pgfonlayer}
\begin{pgfonlayer}{kc}
       \begin{scope}[  
        xshift=2*\xshift, yshift=-30,
             every node/.append style={}]{

            \draw[blue!100,thick] (0,0) rectangle (1,1);
            \filldraw[orange!30, opacity=0.7] (0,0) rectangle (1,1);
            \node at (0.5,0.5) {1};
    

            \draw[blue!100,thick] (0,1) rectangle (1,2);
            \filldraw[orange!30, opacity=0.7] (0,1) rectangle (1,2);
            \node at (0.5,1.5) {2};
    

            \draw[blue!100,thick] (0,2) rectangle (1,3);
            \filldraw[orange!30, opacity=0.7] (0,2) rectangle (1,3);
            \node at (0.5,2.5) {3};
    

            \draw[blue!100,thick] (0,3) rectangle (1,4);
            \filldraw[orange!30, opacity=0.7] (0,3) rectangle (1,4);
            \node at (0.5,3.5) {2};
    

            \draw[blue!100,thick] (0,4) rectangle (1,5);
            \filldraw[orange!30, opacity=0.7] (0,4) rectangle (1,5);
            \node at (0.5,4.5) {1};
    

            \draw[blue!100,thick] (1,0) rectangle (2,1);
            \filldraw[orange!30, opacity=0.7] (1,0) rectangle (2,1);
            \node at (1.5,0.5) {2};
    

            \draw[blue!100,thick] (1,1) rectangle (2,2);
            \filldraw[orange!30, opacity=0.7] (1,1) rectangle (2,2);
            \node at (1.5,1.5) {4};
    

            \draw[blue!100,thick] (1,2) rectangle (2,3);
            \filldraw[orange!30, opacity=0.7] (1,2) rectangle (2,3);
            \node at (1.5,2.5) {6};
    

            \draw[blue!100,thick] (1,3) rectangle (2,4);
            \filldraw[orange!30, opacity=0.7] (1,3) rectangle (2,4);
            \node at (1.5,3.5) {4};
    

            \draw[blue!100,thick] (1,4) rectangle (2,5);
            \filldraw[orange!30, opacity=0.7] (1,4) rectangle (2,5);
            \node at (1.5,4.5) {2};
    

            \draw[blue!100,thick] (2,0) rectangle (3,1);
            \filldraw[orange!30, opacity=0.7] (2,0) rectangle (3,1);
            \node at (2.5,0.5) {3};
    

            \draw[blue!100,thick] (2,1) rectangle (3,2);
            \filldraw[orange!30, opacity=0.7] (2,1) rectangle (3,2);
            \node at (2.5,1.5) {6};
    

            \draw[blue!100,thick] (2,2) rectangle (3,3);
            \filldraw[orange!30, opacity=0.7] (2,2) rectangle (3,3);
            \node at (2.5,2.5) {9};
    

            \draw[blue!100,thick] (2,3) rectangle (3,4);
            \filldraw[orange!30, opacity=0.7] (2,3) rectangle (3,4);
            \node at (2.5,3.5) {6};
    

            \draw[blue!100,thick] (2,4) rectangle (3,5);
            \filldraw[orange!30, opacity=0.7] (2,4) rectangle (3,5);
            \node at (2.5,4.5) {3};
    

            \draw[blue!100,thick] (3,0) rectangle (4,1);
            \filldraw[orange!30, opacity=0.7] (3,0) rectangle (4,1);
            \node at (3.5,0.5) {2};
    

            \draw[blue!100,thick] (3,1) rectangle (4,2);
            \filldraw[orange!30, opacity=0.7] (3,1) rectangle (4,2);
            \node at (3.5,1.5) {4};
    

            \draw[blue!100,thick] (3,2) rectangle (4,3);
            \filldraw[orange!30, opacity=0.7] (3,2) rectangle (4,3);
            \node at (3.5,2.5) {6};
    

            \draw[blue!100,thick] (3,3) rectangle (4,4);
            \filldraw[orange!30, opacity=0.7] (3,3) rectangle (4,4);
            \node at (3.5,3.5) {4};
    

            \draw[blue!100,thick] (3,4) rectangle (4,5);
            \filldraw[orange!30, opacity=0.7] (3,4) rectangle (4,5);
            \node at (3.5,4.5) {2};
    

            \draw[blue!100,thick] (4,0) rectangle (5,1);
            \filldraw[orange!30, opacity=0.7] (4,0) rectangle (5,1);
            \node at (4.5,0.5) {1};
    

            \draw[blue!100,thick] (4,1) rectangle (5,2);
            \filldraw[orange!30, opacity=0.7] (4,1) rectangle (5,2);
            \node at (4.5,1.5) {2};
    

            \draw[blue!100,thick] (4,2) rectangle (5,3);
            \filldraw[orange!30, opacity=0.7] (4,2) rectangle (5,3);
            \node at (4.5,2.5) {3};
    

            \draw[blue!100,thick] (4,3) rectangle (5,4);
            \filldraw[orange!30, opacity=0.7] (4,3) rectangle (5,4);
            \node at (4.5,3.5) {2};
    

            \draw[blue!100,thick] (4,4) rectangle (5,5);
            \filldraw[orange!30, opacity=0.7] (4,4) rectangle (5,5);
            \node at (4.5,4.5) {1};
        \draw[black!100,thick] (0,0) rectangle (5,5);
    }
    \end{scope}
\end{pgfonlayer}
\end{tikzpicture}
}
\caption{An example of two $3\times 3$ convolution operations merged into a single $5\times 5$ convolution operation.}
\label{fig:convfilter}
\end{figure}

==> fig_dp_small.tex <==
\newcommand\tablestructure[4]{
    \def\W{#1}
    \def\H{#2}
    \def\IDID{#3}
    \def\ccc{#4}
    
    \foreach \x in {0,...,\W} {
        \foreach \y in {0,...,\H} {
            \coordinate (\IDID\x\y) at (\xx + \x * \gW, \yy - \y * \gH);
        }   
    }
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID1\H);
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID\W1);
    \foreach \x in {2,...,\W}{
        \foreach \y in {\x,...,\H}{
            \draw ($(\IDID\x\y) + (-\gW, +\gH)$) -- (\IDID\x\y);
        }
    }
    \draw ($(\IDID00) + (0, 0)$) -- ($(\IDID00) + (\gW, -\gH)$);
    \foreach \x in {2,...,\W}{
        \draw ($(\IDID\x0)+ (-\gW,0)$) -- ($(\IDID\x\W)+ (-\gW,0)$);
    }
    \foreach \y in {2,...,\H}{
        \draw ($(\IDID0\y)+ (0,\gH)$) -- ($(\IDID\H\y)+ (0,\gH)$);
    }
}
\newcommand\tablestructureTP[4]{
    \def\W{#1}
    \def\H{#2}
    \def\IDID{#3}
    \def\ccc{#4}
    
    \foreach \y in {0,...,\W} {
        \foreach \x in {0,...,\H} {
            \coordinate (\IDID\y\x) at (\xx + \x * \gW, \yy - \y * \gH);
        }   
    }
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID1\H);
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID\W1);
    \foreach \y in {2,...,\W}{
        \foreach \x in {\y,...,\H}{
            \draw ($(\IDID\y\x) + (-\gW, +\gH)$) -- (\IDID\y\x);
        }
    }
    \draw ($(\IDID00) + (0, 0)$) -- ($(\IDID00) + (\gW, -\gH)$);
    \foreach \y in {2,...,\W}{
        \draw ($(\IDID\y0)+ (0,\gH)$) -- ($(\IDID\y\W)+ (0,\gH)$);
    }
    \foreach \x in {2,...,\H}{
        \draw ($(\IDID0\x)+ (-\gW,0)$) -- ($(\IDID\H\x)+ (-\gW,0)$);
    }
}
\newcommand\putvalue[4]{
\def\i{#1}
\def\j{#2}
\def\CURID{#3}
\def\val{#4}
\node () at ($(\CURID\i\j) + (0.5*\gW, -0.5*\gH)$) {\val};
}
\newcommand\putvaluevdots[4]{
\def\i{#1}
\def\j{#2}
\def\CURID{#3}
\def\val{#4}
\node () at ($(\CURID\i\j) + (0.5*\gW, -0.5*\gH-0.1)$) {\val};
}
\newcommand\putvalueunderline[4]{
\def\i{#1}
\def\j{#2}
\def\CURID{#3}
\def\val{#4}
\node () at ($(\CURID\i\j) + (0.5*\gW, -0.5*\gH-0.04)$) {\val};
}
\newcommand\putvalueTP[4]{
\def\i{#1}
\def\j{#2}
\def\CURID{#3}
\def\val{#4}
\node () at ($(\CURID\j\i) + (0.5*\gW, -0.5*\gH)$) {\val};
}
\newcommand\tablestructureC[4]{
    \def\W{#1}
    \def\H{#2}
    \def\IDID{#3}
    \def\ccc{#4}
    
    \foreach \x in {0,...,\W} {
        \foreach \y in {0,...,\H} {
            \coordinate (\IDID\x\y) at (\xx + \x * \gW, \yy - \y * \gH);
        }   
    }
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID1\H);
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID\W1);
    \draw ($(\IDID00) + (0, 0)$) -- ($(\IDID00) + (\gW, -\gH)$);
    \foreach \x in {2,...,\W}{
        \draw ($(\IDID\x0)+ (-\gW,0)$) -- ($(\IDID\x\H)+ (-\gW,0)$);
    }
    \foreach \y in {2,...,\H}{
        \draw ($(\IDID0\y)+ (0,\gH)$) -- ($(\IDID\W\y)+ (0,\gH)$);
    }
}
\newcommand\tablestructureCTP[4]{
    \def\W{#1}
    \def\H{#2}
    \def\IDID{#3}
    \def\ccc{#4}
    
    \foreach \y in {0,1,2,3} {
        \foreach \x in {0,...,\H} {
            \coordinate (\IDID\y\x) at (\xx + \x * \gW, \yy - \y * \gH);
        }   
    }
    \foreach \y in {4,5} {
        \foreach \x in {0,...,\H} {
            \coordinate (\IDID\y\x) at (\xx + \x * \gW, \yy - \y * \gH-0.4);
        }   
    }
    \foreach \y in {6,7} {
        \foreach \x in {0,...,\H} {
            \coordinate (\IDID\y\x) at (\xx + \x * \gW, \yy - \y * \gH-0.8);
        }   
    }
    \foreach \y in {8,9} {
        \foreach \x in {0,...,\H} {
            \coordinate (\IDID\y\x) at (\xx + \x * \gW, \yy - \y * \gH-1.2);
        }   
    }
    
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID1\H);
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID\W1);
    \draw ($(\IDID00) + (0, 0)$) -- ($(\IDID00) + (\gW, -\gH)$);
    \foreach \y in {1,...,\W}{
        \ifnum\y<\W
        \draw ($(\IDID\y0)$) -- ($(\IDID\y\H)$);
        \fi
    }
    \foreach \x in {2,...,\H}{
        \draw ($(\IDID0\x)+ (-\gW,0)$) -- ($(\IDID\W\x)+ (-\gW,0)$);
    }
}
\newcommand\tableA[2]{
\def\xx{4}
\def\yy{0}
%\tablestructure{5}{5}{A}{green!20}
\tablestructureTP{5}{5}{A}{gray!20}
\putvalue{1}{0}{A}{0}
\putvalue{2}{0}{A}{1}
\putvalue{3}{0}{A}{2}
\putvalue{4}{0}{A}{3}
\putvalue{0}{1}{A}{0}
\putvalue{0}{2}{A}{1}
\putvalue{0}{3}{A}{2}
\putvalue{0}{4}{A}{3}

\putvalue{2}{1}{A}{4}
\putvalue{3}{1}{A}{12}
\putvalue{3}{2}{A}{6}
\putvalue{4}{1}{A}{\textcolor{green!50!black!100}{20}}
\putvalue{4}{2}{A}{\textcolor{blue!80!black!100}{14}}
\putvalue{4}{3}{A}{\textcolor{red}{11}}
}
\newcommand\tableB[2]{
\def\xx{4}
\def\yy{-3.6}
%\tablestructure{5}{5}{B}{blue!15}
\tablestructureTP{5}{5}{B}{gray!20}
\putvalue{1}{0}{B}{0}
\putvalue{2}{0}{B}{1}
\putvalue{3}{0}{B}{2}
\putvalue{4}{0}{B}{3}
\putvalue{0}{1}{B}{0}
\putvalue{0}{2}{B}{1}
\putvalue{0}{3}{B}{2}
\putvalue{0}{4}{B}{3}

\putvalue{2}{1}{B}{0.5}
\putvalue{3}{1}{B}{0.9}
\putvalue{3}{2}{B}{0.3}
\putvalue{4}{1}{B}{\textcolor{green!50!black!100}{1.8}}
\putvalue{4}{2}{B}{\textcolor{blue!80!black!100}{1.4}}
\putvalue{4}{3}{B}{\textcolor{red}{0.7}}
}
\newcommand\tableC[2]{
\def\xx{0}
\def\yy{0}
\tablestructureCTP{9}{5}{C}{red!10}
\putvalueTP{1}{0}{C}{0}
\putvalueTP{2}{0}{C}{1}
\foreach \k in {0,...,4}{
    \ifnum\k>1
    \putvalue{1}{\k}{C}{0}
    \putvalue{2}{\k}{C}{0}
    \fi
    \ifnum\k=1
    \putvalue{1}{1}{C}{0}
    \putvalue{2}{1}{C}{\textcolor{green!50!black!100}{0}}
    \fi
    \putvaluevdots{3}{\k}{C}{$\vdots$}
    \putvaluevdots{5}{\k}{C}{$\vdots$}
    \putvaluevdots{7}{\k}{C}{$\vdots$}
}
\putvalue{1}{0}{C}{0}
\putvalueunderline{2}{0}{C}{\textcolor{green!50!black!100}{\underline{1}}}
\putvalueunderline{4}{0}{C}{\textcolor{blue!80!black!100}{\underline{7}}}
\putvalueunderline{6}{0}{C}{\textcolor{red}{\underline{10}}}
\putvalue{8}{0}{C}{21}
\putvalue{0}{1}{C}{0}
\putvalue{0}{2}{C}{1}
\putvalue{0}{3}{C}{2}
\putvalue{0}{4}{C}{3}

\putvalue{4}{1}{C}{0}
\putvalue{4}{2}{C}{\textcolor{blue!80!black!100}{0.5}}
\putvalue{4}{3}{C}{0}
\putvalue{4}{4}{C}{0}
\putvalue{6}{1}{C}{0}
\putvalue{6}{2}{C}{0.5}
\putvalue{6}{3}{C}{\textcolor{red}{0.8}}
\putvalue{6}{4}{C}{0}
\putvalue{8}{1}{C}{0}
\putvalue{8}{2}{C}{0.5}
\putvalue{8}{3}{C}{0.9}
\putvalue{8}{4}{C}{\textbf{?}}

}
\newcommand\colorrec[2]{
\def\p{#1}
\def\ccc{#2}
\draw[\ccc,line width=2pt] ($(\p)+(1pt, 1pt)$) rectangle ($($(\p)+(\gW, \gH)$) + (-1pt,-1pt)$);
}
\begin{figure}[ht]
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
\def\gW{0.7}
\def\gH{0.6}

\tableA{0}{0}
\tableB{0}{0}
\tableC{0}{0}
\node () at ($(A00) + (0.2*\gW, -0.7*\gH)$) {$l$};
\node () at ($(A00) + (0.7*\gW, -0.25*\gH)$) {$k$};
\node () at ($(B00) + (0.2*\gW, -0.7*\gH)$) {$l$};
\node () at ($(B00) + (0.7*\gW, -0.25*\gH)$) {$k$};
\node () at ($(C00) + (0.2*\gW, -0.7*\gH)$) {$t$};
\node () at ($(C00) + (0.7*\gW, -0.25*\gH)$) {$l$};

%\node () at ($(A20) + (0.5*\gW, 0.5*\gH)$) {\textcolor{green!50!black!100}{$T_\text{opt}[k,l]$}};
\node () at ($(A02) + (0.5*\gW, 0.5*\gH)$) {\textcolor{black}{$T_\text{opt}[k,l]$}};
%\node () at ($(B20) + (0.5*\gW, 0.5*\gH)$) {\textcolor{blue}{$I[k,l]$}};
\node () at ($(B02) + (0.5*\gW, 0.5*\gH)$) {\textcolor{black}{$I[k,l]$}};
\node () at ($(C02) + (0.5*\gW, 0.5*\gH)$) {\textcolor{black}{$D[l,t]$}};

\node () at ($(C60) + (-1.4*\gW, -0.5*\gH-0.015)$) {\footnotesize $\textcolor{red}{\underline{21\!-\!T_\text{opt}[2,3]}}$};
\node () at ($(C40) + (-1.4*\gW, -0.5*\gH-0.015)$) {\footnotesize $\textcolor{blue!80!black!100}{\underline{21\!-\!T_\text{opt}[1,3]}}$};
\node () at ($(C20) + (-1.4*\gW, -0.5*\gH-0.015)$) {\footnotesize $\textcolor{green!50!black!100}{\underline{21\!-\!T_\text{opt}[0,3]}}$};
\colorrec{C31}{green!80!black!100}
\colorrec{C52}{blue}
\colorrec{C73}{red}
\colorrec{C94}{black}
\colorrec{B53}{red}
\colorrec{B52}{blue}
\colorrec{B51}{green!80!black!100}
\colorrec{A53}{red}
\colorrec{A52}{blue}
\colorrec{A51}{green!80!black!100}

\node[align=left,execute at begin node=\setlength{\baselineskip}{1.6em}] () at (3,-7.9) {
$D[3,21]$\\
$= \mathop{\mathrm{max}}\limits_{k'\in\{0,1,2\}}\left(D[k',\underline{21\!-\!T_\text{opt}[k',3]}]+I[k',3]\right)$
\\
$
= ~~~\mathop{\mathrm{max}}~~\{
\textcolor{green!50!black!100}{D[0,\underline{1}] + I[0,3]},
\textcolor{blue!80!black!100}{D[1,\underline{7}] + I[1,3]},
\textcolor{red}{D[2,\underline{10}] + I[2,3]}
\}%=~1.9
$\\
$=~~~~1.9$
};
\draw[line width=2pt] (-1.05,-9.07) rectangle ++(\gW-0.06, \gH-0.06);
% \node[align=left,execute at begin node=\setlength{\baselineskip}{1.6em}] () at (3,-8.7) {
% ~~~~~~~~~~~\,\textcolor{green!50!black!100}{$0~+~1.8$}~~\,\,~~~~~~~~\textcolor{blue!80!black!100}{$0.5~+~1.4$}~~~~~~~~~\,~~~\textcolor{red}{$0.8~+~0.7$}
% };
%\draw[->,line width=1.5pt] (7.70,-8.45+\gH-0.06) to [out=140, in=-40] (C95);
\end{tikzpicture}
}
\caption{Illustration of constructing DP table based on the recurrence relation (\Cref{eq:dprecur}). $D[3, 21]$ (black cell) computes its value upon the solutions of the previous sub-problems ($D[0,1]$, $D[1,7]$, $D[2, 10]$).}
\end{figure}

==> fig_dp_small_new.tex <==
\newcommand\tablestructure[4]{
    \def\W{#1}
    \def\H{#2}
    \def\IDID{#3}
    \def\ccc{#4}
    
    \foreach \x in {0,...,\W} {
        \foreach \y in {0,...,\H} {
            \coordinate (\IDID\x\y) at (\xx + \x * \gW, \yy - \y * \gH);
        }   
    }
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID1\H);
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID\W1);
    \foreach \x in {2,...,\W}{
        \foreach \y in {\x,...,\H}{
            \draw ($(\IDID\x\y) + (-\gW, +\gH)$) -- (\IDID\x\y);
        }
    }
    \draw ($(\IDID00) + (0, 0)$) -- ($(\IDID00) + (\gW, -\gH)$);
    \foreach \x in {2,...,\W}{
        \draw ($(\IDID\x0)+ (-\gW,0)$) -- ($(\IDID\x\W)+ (-\gW,0)$);
    }
    \foreach \y in {2,...,\H}{
        \draw ($(\IDID0\y)+ (0,\gH)$) -- ($(\IDID\H\y)+ (0,\gH)$);
    }
}
\newcommand\tablestructureTP[4]{
    \def\W{#1}
    \def\H{#2}
    \def\IDID{#3}
    \def\ccc{#4}
    
    \foreach \y in {0,...,\W} {
        \foreach \x in {0,...,\H} {
            \coordinate (\IDID\y\x) at (\xx + \x * \gW, \yy - \y * \gH);
        }   
    }
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID1\H);
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID\W1);
    \foreach \y in {2,...,\W}{
        \foreach \x in {\y,...,\H}{
            \draw ($(\IDID\y\x) + (-\gW, +\gH)$) -- (\IDID\y\x);
        }
    }
    \draw ($(\IDID00) + (0, 0)$) -- ($(\IDID00) + (\gW, -\gH)$);
    \foreach \y in {2,...,\W}{
        \draw ($(\IDID\y0)+ (0,\gH)$) -- ($(\IDID\y\W)+ (0,\gH)$);
    }
    \foreach \x in {2,...,\H}{
        \draw ($(\IDID0\x)+ (-\gW,0)$) -- ($(\IDID\H\x)+ (-\gW,0)$);
    }
}
\newcommand\putvalue[4]{
\def\i{#1}
\def\j{#2}
\def\CURID{#3}
\def\val{#4}
\node () at ($(\CURID\i\j) + (0.5*\gW, -0.5*\gH)$) {\val};
}
\newcommand\putvaluevdots[4]{
\def\i{#1}
\def\j{#2}
\def\CURID{#3}
\def\val{#4}
\node () at ($(\CURID\i\j) + (0.5*\gW, -0.5*\gH-0.1)$) {\val};
}
\newcommand\putvalueunderline[4]{
\def\i{#1}
\def\j{#2}
\def\CURID{#3}
\def\val{#4}
\node () at ($(\CURID\i\j) + (0.5*\gW, -0.5*\gH-0.04)$) {\val};
}
\newcommand\putvalueTP[4]{
\def\i{#1}
\def\j{#2}
\def\CURID{#3}
\def\val{#4}
\node () at ($(\CURID\j\i) + (0.5*\gW, -0.5*\gH)$) {\val};
}
\newcommand\tablestructureC[4]{
    \def\W{#1}
    \def\H{#2}
    \def\IDID{#3}
    \def\ccc{#4}
    
    \foreach \x in {0,...,\W} {
        \foreach \y in {0,...,\H} {
            \coordinate (\IDID\x\y) at (\xx + \x * \gW, \yy - \y * \gH);
        }   
    }
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID1\H);
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID\W1);
    \draw ($(\IDID00) + (0, 0)$) -- ($(\IDID00) + (\gW, -\gH)$);
    \foreach \x in {2,...,\W}{
        \draw ($(\IDID\x0)+ (-\gW,0)$) -- ($(\IDID\x\H)+ (-\gW,0)$);
    }
    \foreach \y in {2,...,\H}{
        \draw ($(\IDID0\y)+ (0,\gH)$) -- ($(\IDID\W\y)+ (0,\gH)$);
    }
}
\newcommand\tablestructureCTP[4]{
    \def\W{#1}
    \def\H{#2}
    \def\IDID{#3}
    \def\ccc{#4}
    
    \foreach \y in {0,1,2,3} {
        \foreach \x in {0,...,\H} {
            \coordinate (\IDID\y\x) at (\xx + \x * \gW, \yy - \y * \gH);
        }   
    }
    \foreach \y in {4,5} {
        \foreach \x in {0,...,\H} {
            \coordinate (\IDID\y\x) at (\xx + \x * \gW, \yy - \y * \gH-0.4);
        }   
    }
    \foreach \y in {6,7} {
        \foreach \x in {0,...,\H} {
            \coordinate (\IDID\y\x) at (\xx + \x * \gW, \yy - \y * \gH-0.8);
        }   
    }
    \foreach \y in {8,9} {
        \foreach \x in {0,...,\H} {
            \coordinate (\IDID\y\x) at (\xx + \x * \gW, \yy - \y * \gH-1.2);
        }   
    }
    
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID1\H);
    \draw[fill, \ccc] (\IDID00) rectangle (\IDID\W1);
    \draw ($(\IDID00) + (0, 0)$) -- ($(\IDID00) + (\gW, -\gH)$);
    \foreach \y in {1,...,\W}{
        \ifnum\y<\W
        \draw ($(\IDID\y0)$) -- ($(\IDID\y\H)$);
        \fi
    }
    \foreach \x in {2,...,\H}{
        \draw ($(\IDID0\x)+ (-\gW,0)$) -- ($(\IDID\W\x)+ (-\gW,0)$);
    }
}
\newcommand\tableA[2]{
\def\xx{4}
\def\yy{0}
%\tablestructure{5}{5}{A}{green!20}
\tablestructureTP{5}{5}{A}{gray!20}
\putvalue{1}{0}{A}{0}
\putvalue{2}{0}{A}{1}
\putvalue{3}{0}{A}{2}
\putvalue{4}{0}{A}{3}
\putvalue{0}{1}{A}{0}
\putvalue{0}{2}{A}{1}
\putvalue{0}{3}{A}{2}
\putvalue{0}{4}{A}{3}

\putvalue{2}{1}{A}{4}
\putvalue{3}{1}{A}{12}
\putvalue{3}{2}{A}{6}
\putvalue{4}{1}{A}{\textcolor{green!50!black!100}{20}}
\putvalue{4}{2}{A}{\textcolor{blue!80!black!100}{14}}
\putvalue{4}{3}{A}{\textcolor{red}{11}}
}
\newcommand\tableB[2]{
\def\xx{4}
\def\yy{-3.6}
%\tablestructure{5}{5}{B}{blue!15}
\tablestructureTP{5}{5}{B}{gray!20}
\putvalue{1}{0}{B}{0}
\putvalue{2}{0}{B}{1}
\putvalue{3}{0}{B}{2}
\putvalue{4}{0}{B}{3}
\putvalue{0}{1}{B}{0}
\putvalue{0}{2}{B}{1}
\putvalue{0}{3}{B}{2}
\putvalue{0}{4}{B}{3}

\putvalue{2}{1}{B}{0.5}
\putvalue{3}{1}{B}{0.9}
\putvalue{3}{2}{B}{0.3}
\putvalue{4}{1}{B}{\textcolor{green!50!black!100}{1.8}}
\putvalue{4}{2}{B}{\textcolor{blue!80!black!100}{1.4}}
\putvalue{4}{3}{B}{\textcolor{red}{0.7}}
}
\newcommand\tableC[2]{
\def\xx{0}
\def\yy{0}
\tablestructureCTP{9}{5}{C}{red!10}
\putvalueTP{1}{0}{C}{0}
\putvalueTP{2}{0}{C}{1}
\foreach \k in {0,...,4}{
    \ifnum\k>1
    \putvalue{1}{\k}{C}{0}
    \putvalue{2}{\k}{C}{0}
    \fi
    \ifnum\k=1
    \putvalue{1}{1}{C}{0}
    \putvalue{2}{1}{C}{\textcolor{green!50!black!100}{0}}
    \fi
    \putvaluevdots{3}{\k}{C}{$\vdots$}
    \putvaluevdots{5}{\k}{C}{$\vdots$}
    \putvaluevdots{7}{\k}{C}{$\vdots$}
}
\putvalue{1}{0}{C}{0}
\putvalueunderline{2}{0}{C}{\textcolor{green!50!black!100}{\underline{1}}}
\putvalueunderline{4}{0}{C}{\textcolor{blue!80!black!100}{\underline{7}}}
\putvalueunderline{6}{0}{C}{\textcolor{red}{\underline{10}}}
\putvalue{8}{0}{C}{21}
\putvalue{0}{1}{C}{0}
\putvalue{0}{2}{C}{1}
\putvalue{0}{3}{C}{2}
\putvalue{0}{4}{C}{3}

\putvalue{4}{1}{C}{0}
\putvalue{4}{2}{C}{\textcolor{blue!80!black!100}{0.5}}
\putvalue{4}{3}{C}{0}
\putvalue{4}{4}{C}{0}
\putvalue{6}{1}{C}{0}
\putvalue{6}{2}{C}{0.5}
\putvalue{6}{3}{C}{\textcolor{red}{0.8}}
\putvalue{6}{4}{C}{0}
\putvalue{8}{1}{C}{0}
\putvalue{8}{2}{C}{0.5}
\putvalue{8}{3}{C}{0.9}
\putvalue{8}{4}{C}{\textbf{?}}

}
\newcommand\colorrec[2]{
\def\p{#1}
\def\ccc{#2}
\draw[\ccc,line width=2pt] ($(\p)+(1pt, 1pt)$) rectangle ($($(\p)+(\gW, \gH)$) + (-1pt,-1pt)$);
}
\begin{figure}[ht]
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
\def\gW{0.7}
\def\gH{0.6}

\tableA{0}{0}
\tableB{0}{0}
\tableC{0}{0}
\node () at ($(A00) + (0.2*\gW, -0.7*\gH)$) {$l$};
\node () at ($(A00) + (0.7*\gW, -0.25*\gH)$) {$k$};
\node () at ($(B00) + (0.2*\gW, -0.7*\gH)$) {$l$};
\node () at ($(B00) + (0.7*\gW, -0.25*\gH)$) {$k$};
\node () at ($(C00) + (0.2*\gW, -0.7*\gH)$) {$t$};
\node () at ($(C00) + (0.7*\gW, -0.25*\gH)$) {$l$};

%\node () at ($(A20) + (0.5*\gW, 0.5*\gH)$) {\textcolor{green!50!black!100}{$T_\text{opt}[k,l]$}};
\node () at ($(A02) + (0.5*\gW, 0.5*\gH)$) {\textcolor{black}{$T_\text{opt}[k,l]$}};
%\node () at ($(B20) + (0.5*\gW, 0.5*\gH)$) {\textcolor{blue}{$I[k,l]$}};
\node () at ($(B02) + (0.5*\gW, 0.5*\gH)$) {\textcolor{black}{$I[k,l]$}};
\node () at ($(C02) + (0.5*\gW, 0.5*\gH)$) {\textcolor{black}{$D[l,t]$}};

\node () at ($(C60) + (-1.4*\gW, -0.5*\gH-0.015)$) {\footnotesize $\textcolor{red}{\underline{21\!-\!T_\text{opt}[2,3]}}$};
\node () at ($(C40) + (-1.4*\gW, -0.5*\gH-0.015)$) {\footnotesize $\textcolor{blue!80!black!100}{\underline{21\!-\!T_\text{opt}[1,3]}}$};
\node () at ($(C20) + (-1.4*\gW, -0.5*\gH-0.015)$) {\footnotesize $\textcolor{green!50!black!100}{\underline{21\!-\!T_\text{opt}[0,3]}}$};
\colorrec{C31}{green!80!black!100}
\colorrec{C52}{blue}
\colorrec{C73}{red}
\colorrec{C94}{black}
\colorrec{B53}{red}
\colorrec{B52}{blue}
\colorrec{B51}{green!80!black!100}
\colorrec{A53}{red}
\colorrec{A52}{blue}
\colorrec{A51}{green!80!black!100}

% \node[align=left,execute at begin node=\setlength{\baselineskip}{1.6em}] () at (3,-7.9) {
% $D[3,21]$\\
% $= \mathop{\mathrm{max}}\limits_{k'\in\{0,1,2\}}\left(D[k',\underline{21\!-\!T_\text{opt}[k',3]}]+I[k',3]\right)$
% \\
% $
% = ~~~\mathop{\mathrm{max}}~~\{
% \textcolor{green!50!black!100}{D[0,\underline{1}] + I[0,3]},
% \textcolor{blue!80!black!100}{D[1,\underline{7}] + I[1,3]},
% \textcolor{red}{D[2,\underline{10}] + I[2,3]}
% \}%=~1.9
% $\\
% $=~~~~1.9$
% };
% \draw[line width=2pt] (-1.05,-9.07) rectangle ++(\gW-0.06, \gH-0.06);
% % \node[align=left,execute at begin node=\setlength{\baselineskip}{1.6em}] () at (3,-8.7) {
% % ~~~~~~~~~~~\,\textcolor{green!50!black!100}{$0~+~1.8$}~~\,\,~~~~~~~~\textcolor{blue!80!black!100}{$0.5~+~1.4$}~~~~~~~~~\,~~~\textcolor{red}{$0.8~+~0.7$}
% % };
% %\draw[->,line width=1.5pt] (7.70,-8.45+\gH-0.06) to [out=140, in=-40] (C95);
% \node (M) at (-1.6, -9.7) {\large $X$};
% \node (X) at (-0.3, -9.7) {\large $f_{\theta_1}$};
% \node (Y) at (1.0, -9.7) {\large $\sigma_1$};
% \node (Z) at (2.3, -9.7) {\large $f_{\theta_2}$};
% \node (W) at (3.6, -9.7) {\large $\mathrm{id}$};
% \node (V) at (4.9, -9.7) {\large $f_{\theta_3}$};
% \node (U) at (6.2, -9.7) {\large $\sigma_3$};
% \node (T) at (7.5, -9.7) {};
% \node[black!100] () at ($($(M)!0.5!(X)$) + (0,0)$) {$\rightarrow$};
% \node[black!100] () at ($($(X)!0.5!(Y)$) + (0,0)$) {$\rightarrow$};
% \node[black!100] () at ($($(Y)!0.5!(Z)$) + (0,0)$) {$\rightarrow$};
% \node[black!100] () at ($($(Z)!0.5!(W)$) + (0,0)$) {$\rightarrow$};
% \node[black!100] () at ($($(W)!0.5!(V)$) + (0,0)$) {$\rightarrow$};
% \node[black!100] () at ($($(V)!0.5!(U)$) + (0,0)$) {$\rightarrow$};
% \node[black!100] () at ($($(U)!0.5!(T)$) + (0,0)$) {$\rightarrow$};
% \node[black!100] () at ($(T) + (0,0)$) {$\cdots$};
% \draw[rounded corners,line width=0.3mm,inner sep=20pt, blue!80!black!100] ($(X) + (-0.3,-0.4)$) rectangle  ($(Y) + (0.3,0.4)$);
% \draw[rounded corners,line width=0.3mm,inner sep=20pt, blue!80!black!100] ($(Z) + (-0.3,-0.4)$) rectangle  ($(U) + (0.3,0.4)$);
%         %\draw[rounded corners, dash pattern=on 6pt off 6pt,line width=0.5mm,inner sep=20pt, black!100] ($(B160)+(1.0,-0.4)$) rectangle ($(B110)+(-0.2,1.5)$) {};
% \node[black!100] () at ($($(Y)!0.5!(Z)$) + (-1.5,-0.8)$) {$A[3,21]~=~\textcolor{blue!80!black!100}{A[1,
% \underline{7}] + \{1\}}$};


\node[align=left,execute at begin node=\setlength{\baselineskip}{1.6em}] () at (3,-7.4) {
$D[3,21]$\\
$
~~= \mathop{\mathrm{max}}~~\{
\textcolor{green!50!black!100}{D[0,\underline{1}] + I[0,3]},
\textcolor{blue!80!black!100}{D[1,\underline{7}] + I[1,3]},
\textcolor{red}{D[2,\underline{10}] + I[2,3]}
\}%=~1.9
$\\
$~~=~1.9$
};
\draw[line width=2pt] (-1.02,-8.26) rectangle ++(\gW-0.06, \gH-0.06);
% \node[align=left,execute at begin node=\setlength{\baselineskip}{1.6em}] () at (3,-8.7) {
% ~~~~~~~~~~~\,\textcolor{green!50!black!100}{$0~+~1.8$}~~\,\,~~~~~~~~\textcolor{blue!80!black!100}{$0.5~+~1.4$}~~~~~~~~~\,~~~\textcolor{red}{$0.8~+~0.7$}
% };
%\draw[->,line width=1.5pt] (7.70,-8.45+\gH-0.06) to [out=140, in=-40] (C95);
\node (M) at (-1.6, -8.85) {\large $X$};
\node (X) at (-0.3, -8.85) {\large $f_{\theta_1}$};
\node (Y) at (1.0, -8.85) {\large $\sigma_1$};
\node (Z) at (2.3, -8.85) {\large $f_{\theta_2}$};
\node (W) at (3.6, -8.85) {\large $\mathrm{id}$};
\node (V) at (4.9, -8.85) {\large $f_{\theta_3}$};
\node (U) at (6.2, -8.85) {\large $\sigma_3$};
\node (T) at (7.5, -8.85) {};
\node[black!100] () at ($($(M)!0.5!(X)$) + (0,0)$) {$\rightarrow$};
\node[black!100] () at ($($(X)!0.5!(Y)$) + (0,0)$) {$\rightarrow$};
\node[black!100] () at ($($(Y)!0.5!(Z)$) + (0,0)$) {$\rightarrow$};
\node[black!100] () at ($($(Z)!0.5!(W)$) + (0,0)$) {$\rightarrow$};
\node[black!100] () at ($($(W)!0.5!(V)$) + (0,0)$) {$\rightarrow$};
\node[black!100] () at ($($(V)!0.5!(U)$) + (0,0)$) {$\rightarrow$};
\node[black!100] () at ($($(U)!0.5!(T)$) + (0,0)$) {$\rightarrow$};
\node[black!100] () at ($(T) + (0,0)$) {$\cdots$};
\draw[rounded corners,line width=0.3mm,inner sep=20pt, blue!80!black!100] ($(X) + (-0.3,-0.4)$) rectangle  ($(Y) + (0.3,0.4)$);
\draw[rounded corners,line width=0.3mm,inner sep=20pt, blue!80!black!100] ($(Z) + (-0.3,-0.4)$) rectangle  ($(U) + (0.3,0.4)$);
        %\draw[rounded corners, dash pattern=on 6pt off 6pt,line width=0.5mm,inner sep=20pt, black!100] ($(B160)+(1.0,-0.4)$) rectangle ($(B110)+(-0.2,1.5)$) {};
\node[black!100] () at ($($(Y)!0.5!(Z)$) + (-1.45,-0.8)$) {$A[3,21]~=~\textcolor{blue!80!black!100}{A[1,
\underline{7}] \cup \{1\}}$};
\end{tikzpicture}
}
\caption{Illustration of constructing DP table based on the recurrence relation (\Cref{eq:dprecur}). $D[3, 21]$ (black cell) computes its value upon the solutions of the previous sub-problems ($D[0,1]$, $D[1,7]$, $D[2, 10]$).}
\end{figure}

==> fig_main2.tex <==
% \documentclass{article}
% \usepackage[utf8]{inputenc}
% \usepackage{tikz}
% \usepackage[margin=0.5in]{geometry}
% %\documentclass[landscape, 12pt]{report}
% %\usepackage[landscape]{geometry}
% \usepackage{graphicx}
% \usepackage{hyperref}
% \usepackage{url}
% \usepackage{amssymb,amsmath,amsthm}
% \usepackage{tikz}
% \usepackage{tkz-tab}
% \usepackage{adjustbox}
% \usepackage{pgfplots}
% \usepackage{subcaption}

% \usepackage{enumitem}
% \usepackage{verbatim}
% \usepackage{multirow}
% \usepackage{algorithm,algorithmic}
% \usetikzlibrary{positioning,decorations.pathreplacing,decorations.markings,calc,arrows,hobby,backgrounds,patterns}
\newcommand\grid[3]{
    \def\p{#1}
    \def\xx{#2}
    \def\yy{#3}
  \draw[fill,\c,opacity=0.9] (\p) rectangle ++(\xx,\yy);
  \draw[gray!60] ($(\p) + (\xx/3,0)$) -- ($(\p) + (\xx/3,\yy)$);
  \draw[gray!60] ($(\p) + (\xx/3*2,0)$) -- ($(\p) + (\xx/3*2,\yy)$);
  \draw[gray!60] ($(\p) + (0,\yy/3)$) -- ($(\p) + (\xx,\yy/3)$);
  \draw[gray!60] ($(\p) + (0,\yy/3*2)$) -- ($(\p) + (\xx,\yy/3*2)$);
  \draw (\p) rectangle ++(\xx,\yy);
}
\newcommand\gridd[3]{
    \def\p{#1}
    \def\xx{#2}
    \def\yy{#3}
  \draw[fill,\c,opacity=0.9] (\p) rectangle ++(\xx,\yy);
  \draw[gray!60] ($(\p) + (\xx/5,0)$) -- ($(\p) + (\xx/5,\yy)$);
  \draw[gray!60] ($(\p) + (\xx/5*2,0)$) -- ($(\p) + (\xx/5*2,\yy)$);
  \draw[gray!60] ($(\p) + (\xx/5*3,0)$) -- ($(\p) + (\xx/5*3,\yy)$);
  \draw[gray!60] ($(\p) + (\xx/5*4,0)$) -- ($(\p) + (\xx/5*4,\yy)$);
  \draw[gray!60] ($(\p) + (0,\yy/5)$) -- ($(\p) + (\xx,\yy/5)$);
  \draw[gray!60] ($(\p) + (0,\yy/5*2)$) -- ($(\p) + (\xx,\yy/5*2)$);
  \draw[gray!60] ($(\p) + (0,\yy/5*3)$) -- ($(\p) + (\xx,\yy/5*3)$);
  \draw[gray!60] ($(\p) + (0,\yy/5*4)$) -- ($(\p) + (\xx,\yy/5*4)$);
  \draw (\p) rectangle ++(\xx,\yy);
}
\newcommand\griddd[3]{
    \def\p{#1}
    \def\xx{#2}
    \def\yy{#3}
  \draw[fill,\c,opacity=0.9] (\p) rectangle ++(\xx,\yy);
  \draw[gray!60] ($(\p) + (\xx/7,0)$) -- ($(\p) + (\xx/7,\yy)$);
  \draw[gray!60] ($(\p) + (\xx/7*2,0)$) -- ($(\p) + (\xx/7*2,\yy)$);
  \draw[gray!60] ($(\p) + (\xx/7*3,0)$) -- ($(\p) + (\xx/7*3,\yy)$);
  \draw[gray!60] ($(\p) + (\xx/7*4,0)$) -- ($(\p) + (\xx/7*4,\yy)$);
  \draw[gray!60] ($(\p) + (\xx/7*5,0)$) -- ($(\p) + (\xx/7*5,\yy)$);
  \draw[gray!60] ($(\p) + (\xx/7*6,0)$) -- ($(\p) + (\xx/7*6,\yy)$);
  \draw[gray!60] ($(\p) + (0,\yy/7)$) -- ($(\p) + (\xx,\yy/7)$);
  \draw[gray!60] ($(\p) + (0,\yy/7*2)$) -- ($(\p) + (\xx,\yy/7*2)$);
  \draw[gray!60] ($(\p) + (0,\yy/7*3)$) -- ($(\p) + (\xx,\yy/7*3)$);
  \draw[gray!60] ($(\p) + (0,\yy/7*4)$) -- ($(\p) + (\xx,\yy/7*4)$);
  \draw[gray!60] ($(\p) + (0,\yy/7*5)$) -- ($(\p) + (\xx,\yy/7*5)$);
  \draw[gray!60] ($(\p) + (0,\yy/7*6)$) -- ($(\p) + (\xx,\yy/7*6)$);
  \draw (\p) rectangle ++(\xx,\yy);
}

\newcommand\fm[5]{
    \def\nin{#1}
    \def\convid{#2}
    \def\xx{#3}
    \def\yy{#4}
    \def\ccc{#5}
        \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={1*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \coordinate (A\convid\i) at (\xx,\yy);
              \coordinate (DA\convid\i) at ($(\xx,\yy)+(\fmw,\fmh)$);
        \end{scope}
        }
    \draw[\ccc] (A\convid0) -- (A\convid\nin);
    \draw[\ccc] ($(A\convid0) + (\fmw,0)$) -- ($(A\convid\nin) + (\fmw,0)$);
    \draw[\ccc] (DA\convid0) -- (DA\convid\nin);
        \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={1.5*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[fill,\ccc,opacity=0.9] (A\convid\i) rectangle ++(\fmw,\fmh);
              \ifnum\i=0
              \draw[red!40] (A\convid\i) rectangle ++(\fmw,\fmh);
              \else
            \ifnum\i=\nin
              \draw (A\convid\i) rectangle ++(\fmw,\fmh);            
            \else 
              \draw[red!40] (A\convid\i) rectangle ++(\fmw,\fmh);           
            \fi
            \fi
        \end{scope}
        }
    \draw[fill,\ccc,opacity=0.8] (A\convid0) -- (A\convid\nin) -- ($(A\convid\nin)+(\fmw,0)$) -- ($(A\convid0)+(\fmw,0)$) --cycle; 
    \draw[fill,\ccc,opacity=0.8] (DA\convid0) -- (DA\convid\nin) -- ($(A\convid\nin)+(\fmw,0)$) -- ($(A\convid0)+(\fmw,0)$) --cycle; 
    \draw[black] (DA\convid0) -- (DA\convid\nin) -- ($(A\convid\nin)+(\fmw,0)$) -- ($(A\convid0)+(\fmw,0)$) --cycle; 
    \draw[black] (A\convid0) -- (A\convid\nin) -- ($(A\convid\nin)+(\fmw,0)$) -- ($(A\convid0)+(\fmw,0)$) --cycle; 
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={1.5*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[red!80!black!60] ($(A\convid\i)+(\fmw,0)$) -- ($(A\convid\i)+(\fmw,\fmh)$);
              \draw[red!80!black!60] (A\convid\i) -- ($(A\convid\i)+(\fmw,0.0)$);
        \end{scope}
        }
        \begin{scope}[  % Lower layer
            yshift={-100},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[black] ($(A\convid\nin)+(\fmw,0)$) -- ($(A\convid\nin)+(\fmw,\fmh)$);
              \draw[black] (A\convid\nin) -- ($(A\convid\nin)+(\fmw,0.0)$);
              \draw[black] ($(A\convid0)+(\fmw,0)$) -- ($(A\convid0)+(\fmw,\fmh)$);
              \draw[black] (A\convid0) -- ($(A\convid0)+(\fmw,0.0)$);
        \end{scope}
}
\newcommand\gfm[5]{
    \def\nin{#1}
    \def\convid{#2}
    \def\xx{#3}
    \def\yy{#4}
    \def\ccc{green!20}
        \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={1*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \coordinate (A\convid\i) at (\xx,\yy);
              \coordinate (DA\convid\i) at ($(\xx,\yy)+(1,0.7)$);
        \end{scope}
        }
    \draw[\ccc] (A\convid0) -- (A\convid\nin);
    \draw[\ccc] ($(A\convid0) + (1,0)$) -- ($(A\convid\nin) + (1,0)$);
    \draw[\ccc] (DA\convid0) -- (DA\convid\nin);
        \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={1.5*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[fill,\ccc,opacity=0.9] (A\convid\i) rectangle ++(1,0.7);
              \ifnum\i=0
              %\draw[green!60] (A\convid\i) rectangle ++(1,0.7);
              \draw[black] (A\convid\i) rectangle ++(1,0.7);
              \else
            \ifnum\i=\nin
              \draw (A\convid\i) rectangle ++(1,0.7);            
            \else 
              %\draw[green!60] (A\convid\i) rectangle ++(1,0.7);           
              \draw[green!60] (A\convid\i) rectangle ++(1,0.7);           
            \fi
            \fi
        \end{scope}
        }
    \draw[fill,\ccc,opacity=0.9] (A\convid0) -- (A\convid\nin) -- ($(A\convid\nin)+(1,0)$) -- ($(A\convid0)+(1,0)$) --cycle; 
    \draw[fill,\ccc,opacity=0.9] (DA\convid0) -- (DA\convid\nin) -- ($(A\convid\nin)+(1,0)$) -- ($(A\convid0)+(1,0)$) --cycle; 
    \draw[black] (DA\convid0) -- (DA\convid\nin) -- ($(A\convid\nin)+(1,0)$) -- ($(A\convid0)+(1,0)$) --cycle; 
    \draw[black] (A\convid0) -- (A\convid\nin) -- ($(A\convid\nin)+(1,0)$) -- ($(A\convid0)+(1,0)$) --cycle; 
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={1.5*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              %\draw[green!80!black!100] ($(A\convid\i)+(1,0)$) -- ($(A\convid\i)+(1,0.7)$);
              \draw[green!80!black!100] ($(A\convid\i)+(1,0)$) -- ($(A\convid\i)+(1,0.7)$);
              %\draw[green!80!black!100] (A\convid\i) -- ($(A\convid\i)+(1,0.0)$);
              \draw[green!80!black!100] (A\convid\i) -- ($(A\convid\i)+(1,0.0)$);
        \end{scope}
        }
        \begin{scope}[  % Lower layer
            yshift={-100},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[black] ($(A\convid\nin)+(1,0)$) -- ($(A\convid\nin)+(1,0.7)$);
              \draw[black] (A\convid\nin) -- ($(A\convid\nin)+(1,0.0)$);
              \draw[black] ($(A\convid0)+(1,0)$) -- ($(A\convid0)+(1,0.7)$);
              \draw[black] (A\convid0) -- ($(A\convid0)+(1,0.0)$);
        \end{scope}
}

\newcommand\whitefm[5]{
    \def\nin{#1}
    \def\convid{#2}
    \def\xx{#3}
    \def\yy{#4}
    \def\marg{#5}
    \def\ccc{green!20}
        \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={\marg+1*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \coordinate (A\convid\i) at (\xx,\yy);
              \coordinate (DA\convid\i) at ($(\xx,\yy)+(1,0.7)$);
        \end{scope}
        }
    \draw[\ccc] (A\convid0) -- (A\convid\nin);
    \draw[\ccc] ($(A\convid0) + (1,0)$) -- ($(A\convid\nin) + (1,0)$);
    \draw[\ccc] (DA\convid0) -- (DA\convid\nin);
        \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={\marg+1*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[fill,\ccc,opacity=0.9] (A\convid\i) rectangle ++(1,0.7);
              \ifnum\i=0
              %\draw[green!60] (A\convid\i) rectangle ++(1,0.7);
              \draw[black] (A\convid\i) rectangle ++(1,0.7);
              \else
            \ifnum\i=\nin
              \draw (A\convid\i) rectangle ++(1,0.7);            
            \else 
              %\draw[green!60] (A\convid\i) rectangle ++(1,0.7);           
              \draw[green!60] (A\convid\i) rectangle ++(1,0.7);           
            \fi
            \fi
        \end{scope}
        }
    \draw[fill,\ccc,opacity=0.9] (A\convid0) -- (A\convid\nin) -- ($(A\convid\nin)+(1,0)$) -- ($(A\convid0)+(1,0)$) --cycle; 
    \draw[fill,\ccc,opacity=0.9] (DA\convid0) -- (DA\convid\nin) -- ($(A\convid\nin)+(1,0)$) -- ($(A\convid0)+(1,0)$) --cycle; 
    \draw[black] (DA\convid0) -- (DA\convid\nin) -- ($(A\convid\nin)+(1,0)$) -- ($(A\convid0)+(1,0)$) --cycle; 
    \draw[black] (A\convid0) -- (A\convid\nin) -- ($(A\convid\nin)+(1,0)$) -- ($(A\convid0)+(1,0)$) --cycle; 
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={\marg},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              %\draw[green!80!black!100] ($(A\convid\i)+(1,0)$) -- ($(A\convid\i)+(1,0.7)$);
              \draw[green!80!black!100] ($(A\convid\i)+(1,0)$) -- ($(A\convid\i)+(1,0.7)$);
              %\draw[green!80!black!100] (A\convid\i) -- ($(A\convid\i)+(1,0.0)$);
              \draw[green!80!black!100] (A\convid\i) -- ($(A\convid\i)+(1,0.0)$);
        \end{scope}
        }
        \begin{scope}[  % Lower layer
            yshift={\marg},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[black] ($(A\convid\nin)+(1,0)$) -- ($(A\convid\nin)+(1,0.7)$);
              \draw[black] (A\convid\nin) -- ($(A\convid\nin)+(1,0.0)$);
              \draw[black] ($(A\convid0)+(1,0)$) -- ($(A\convid0)+(1,0.7)$);
              \draw[black] (A\convid0) -- ($(A\convid0)+(1,0.0)$);
        \end{scope}
}
\newcommand\bfm[5]{
    \def\nin{#1}
    \def\convid{#2}
    \def\xx{#3}
    \def\yy{#4}
    \def\ccc{#5}
        \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={-100+1*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \coordinate (BA\convid\i) at (\xx,\yy);
              \coordinate (DBA\convid\i) at ($(\xx,\yy)+(1,0.7)$);
        \end{scope}
        }
    \draw[\ccc] (BA\convid0) -- (BA\convid\nin);
    \draw[\ccc] ($(BA\convid0) + (1,0)$) -- ($(BA\convid\nin) + (1,0)$);
    \draw[\ccc] (DBA\convid0) -- (DBA\convid\nin);
        \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={-100+1.5*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[fill,\ccc,opacity=0.9] (BA\convid\i) rectangle ++(1,0.7);
              \ifnum\i=0
              \draw[red!40] (BA\convid\i) rectangle ++(1,0.7);
              \else
            \ifnum\i=\nin
              \draw (BA\convid\i) rectangle ++(1,0.7);            
            \else 
              \draw[red!40] (BA\convid\i) rectangle ++(1,0.7);           
            \fi
            \fi
        \end{scope}
        }
    \draw[fill,\ccc,opacity=0.8] (BA\convid0) -- (BA\convid\nin) -- ($(BA\convid\nin)+(1,0)$) -- ($(BA\convid0)+(1,0)$) --cycle; 
    \draw[fill,\ccc,opacity=0.8] (DBA\convid0) -- (DBA\convid\nin) -- ($(BA\convid\nin)+(1,0)$) -- ($(BA\convid0)+(1,0)$) --cycle; 
    \draw[black] (DBA\convid0) -- (DBA\convid\nin) -- ($(BA\convid\nin)+(1,0)$) -- ($(BA\convid0)+(1,0)$) --cycle; 
    \draw[black] (BA\convid0) -- (BA\convid\nin) -- ($(BA\convid\nin)+(1,0)$) -- ($(BA\convid0)+(1,0)$) --cycle; 
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={-100+1.5*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[red!80!black!60] ($(BA\convid\i)+(1,0)$) -- ($(BA\convid\i)+(1,0.7)$);
              \draw[red!80!black!60] (BA\convid\i) -- ($(BA\convid\i)+(1,0.0)$);
        \end{scope}
        }
        \begin{scope}[  % Lower layer
            yshift={-100},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[black] ($(BA\convid\nin)+(1,0)$) -- ($(BA\convid\nin)+(1,0.7)$);
              \draw[black] (BA\convid\nin) -- ($(BA\convid\nin)+(1,0.0)$);
              \draw[black] ($(BA\convid0)+(1,0)$) -- ($(BA\convid0)+(1,0.7)$);
              \draw[black] (BA\convid0) -- ($(BA\convid0)+(1,0.0)$);
        \end{scope}
}

\newcommand\ffm[5]{
    \def\nin{#1}
    \def\convid{#2}
    \def\xx{#3}
    \def\yy{#4}
    \def\ccc{#5}
        \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={100+1*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \coordinate (BA\convid\i) at (\xx,\yy);
              \coordinate (DBA\convid\i) at ($(\xx,\yy)+(1,0.7)$);
        \end{scope}
        }
    \draw[\ccc] (BA\convid0) -- (BA\convid\nin);
    \draw[\ccc] ($(BA\convid0) + (1,0)$) -- ($(BA\convid\nin) + (1,0)$);
    \draw[\ccc] (DBA\convid0) -- (DBA\convid\nin);
        \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={100+1.5*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[fill,\ccc,opacity=0.9] (BA\convid\i) rectangle ++(1,0.7);
              \ifnum\i=0
              \draw[red!40] (BA\convid\i) rectangle ++(1,0.7);
              \else
            \ifnum\i=\nin
              \draw (BA\convid\i) rectangle ++(1,0.7);            
            \else 
              \draw[red!40] (BA\convid\i) rectangle ++(1,0.7);           
            \fi
            \fi
        \end{scope}
        }
    \draw[fill,\ccc,opacity=0.8] (BA\convid0) -- (BA\convid\nin) -- ($(BA\convid\nin)+(1,0)$) -- ($(BA\convid0)+(1,0)$) --cycle; 
    \draw[fill,\ccc,opacity=0.8] (DBA\convid0) -- (DBA\convid\nin) -- ($(BA\convid\nin)+(1,0)$) -- ($(BA\convid0)+(1,0)$) --cycle; 
    \draw[black] (DBA\convid0) -- (DBA\convid\nin) -- ($(BA\convid\nin)+(1,0)$) -- ($(BA\convid0)+(1,0)$) --cycle; 
    \draw[black] (BA\convid0) -- (BA\convid\nin) -- ($(BA\convid\nin)+(1,0)$) -- ($(BA\convid0)+(1,0)$) --cycle; 
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={100+1.5*\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[red!80!black!60] ($(BA\convid\i)+(1,0)$) -- ($(BA\convid\i)+(1,0.7)$);
              \draw[red!80!black!60] (BA\convid\i) -- ($(BA\convid\i)+(1,0.0)$);
        \end{scope}
        }
        \begin{scope}[  % Lower layer
            yshift={100},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
              \draw[black] ($(BA\convid\nin)+(1,0)$) -- ($(BA\convid\nin)+(1,0.7)$);
              \draw[black] (BA\convid\nin) -- ($(BA\convid\nin)+(1,0.0)$);
              \draw[black] ($(BA\convid0)+(1,0)$) -- ($(BA\convid0)+(1,0.7)$);
              \draw[black] (BA\convid0) -- ($(BA\convid0)+(1,0.0)$);
        \end{scope}
}
\newcommand\bbconv[4]{
    \def\nin{#1}
    \def\convid{#2}
    \def\xx{#3}
    \def\yy{#4}
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
                \coordinate (B\convid\i) at ($(\xx,\yy)+(0,0)$);
                \coordinate (DB\convid\i) at ($(\xx,\yy)+(0.3,0.21)$);
              \grid{B\convid\i}{0.3}{0.21}
        \end{scope}
    }

    \draw[fill,gray!10,opacity=0.8] (B\convid0) -- (B\convid\nin) -- ($(B\convid\nin)+(0.3,0)$) -- ($(B\convid0)+(0.3,0)$) --cycle; 
    \draw[fill,gray!10,opacity=0.8] (DB\convid0) -- (DB\convid\nin) -- ($(B\convid\nin)+(0.3,0)$) -- ($(B\convid0)+(0.3,0)$) --cycle; 
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
            \draw[gray!80] (B\convid\i) -- ($(B\convid\i)+(0.3,0)$);
            \draw[gray!80] (DB\convid\i) -- ($(B\convid\i)+(0.3,0)$);
        \end{scope}
    }
    \draw[black] (B\convid0) -- (B\convid\nin) -- ($(B\convid\nin)+(0.3,0)$) -- ($(B\convid0)+(0.3,0)$) --cycle; 
    \draw[black] (DB\convid0) -- (DB\convid\nin) -- ($(B\convid\nin)+(0.3,0)$) -- ($(B\convid0)+(0.3,0)$) --cycle;
    % \draw[gray!60] ($(B\convid0) + (0.5/3,0)$) -- ($(B\convid\nin) + (0.5/3,0)$) ;
    % \draw[gray!60] ($(B\convid0) + (0.5/3*2,0)$) -- ($(B\convid\nin) + (0.5/3*2,0)$) ;

    % \draw[gray!60] ($(DB\convid0)!0.333333!(B\convid0) + (0.5/3,0)$) -- ($(DB\convid\nin)!0.333333!(B\convid\nin) + (0.5/3,0)$);
    % \draw[gray!60] ($(DB\convid0)!0.666667!(B\convid0) + (0.5/3*2,0)$) -- ($(DB\convid\nin)!0.666667!(B\convid\nin) + (0.5/3*2,0)$);
}

\newcommand\bconv[4]{
    \def\nin{#1}
    \def\convid{#2}
    \def\xx{#3}
    \def\yy{#4}
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={-100+\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
                \coordinate (EB\convid\i) at ($(\xx,\yy)+(0,0)$);
                \coordinate (DEB\convid\i) at ($(\xx,\yy)+(0.3,0.21)$);
              \grid{EB\convid\i}{0.3}{0.21}
        \end{scope}
    }

    \draw[fill,gray!10,opacity=0.8] (EB\convid0) -- (EB\convid\nin) -- ($(EB\convid\nin)+(0.3,0)$) -- ($(EB\convid0)+(0.3,0)$) --cycle; 
    \draw[fill,gray!10,opacity=0.8] (DEB\convid0) -- (DEB\convid\nin) -- ($(EB\convid\nin)+(0.3,0)$) -- ($(EB\convid0)+(0.3,0)$) --cycle; 
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={-100+\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
            \draw[gray!80] (EB\convid\i) -- ($(EB\convid\i)+(0.3,0)$);
            \draw[gray!80] (DEB\convid\i) -- ($(EB\convid\i)+(0.3,0)$);
        \end{scope}
    }
    \draw[black] (EB\convid0) -- (EB\convid\nin) -- ($(EB\convid\nin)+(0.3,0)$) -- ($(EB\convid0)+(0.3,0)$) --cycle; 
    \draw[black] (DEB\convid0) -- (DEB\convid\nin) -- ($(EB\convid\nin)+(0.3,0)$) -- ($(EB\convid0)+(0.3,0)$) --cycle; 
    
    \draw[black] (EB\convid0) -- (EB\convid\nin) -- ($(EB\convid\nin)+(0.3,0)$) -- ($(EB\convid0)+(0.3,0)$) --cycle; 
    \draw[black] (DEB\convid0) -- (DEB\convid\nin) -- ($(EB\convid\nin)+(0.3,0)$) -- ($(EB\convid0)+(0.3,0)$) --cycle;
    % \draw[gray!60] ($(EB\convid0) + (0.5/3,0)$) -- ($(EB\convid\nin) + (0.5/3,0)$) ;
    % \draw[gray!60] ($(EB\convid0) + (0.5/3*2,0)$) -- ($(EB\convid\nin) + (0.5/3*2,0)$) ;

    % \draw[gray!60] ($(DEB\convid0)!0.333333!(EB\convid0) + (0.5/3,0)$) -- ($(DEB\convid\nin)!0.333333!(EB\convid\nin) + (0.5/3,0)$);
    % \draw[gray!60] ($(DEB\convid0)!0.666667!(EB\convid0) + (0.5/3*2,0)$) -- ($(DEB\convid\nin)!0.666667!(EB\convid\nin) + (0.5/3*2,0)$);
}
% \newcommand\bconvv[4]{
%     \def\nin{#1}
%     \def\convid{#2}
%     \def\xx{#3}
%     \def\yy{#4}
%     \foreach \i in {0,1,...,\nin} {
%         \begin{scope}[  % Lower layer
%             yshift={-70+\channelwidth*\i},every node/.append style={
%                  yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
%               ]              
%                 \coordinate (B\convid\i) at ($(\xx,\yy)+(0,0)$);
%               \gridd{B\convid\i}{0.5*5/3}{0.35*5/3}
%         \end{scope}
%     }
% }

\newcommand\bconvv[4]{
    \def\nin{#1}
    \def\convid{#2}
    \def\xx{#3}
    \def\yy{#4}
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={-100+\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
                \coordinate (EB\convid\i) at ($(\xx,\yy)+(0,0)$);
                \coordinate (DEB\convid\i) at ($(\xx,\yy)+(0.3*5/3,0.21*5/3)$);
              \gridd{EB\convid\i}{0.3*5/3}{0.21*5/3}
        \end{scope}
    }

    \draw[fill,gray!10,opacity=0.8] (EB\convid0) -- (EB\convid\nin) -- ($(EB\convid\nin)+(0.3*5/3,0)$) -- ($(EB\convid0)+(0.3*5/3,0)$) --cycle; 
    \draw[fill,gray!10,opacity=0.8] (DEB\convid0) -- (DEB\convid\nin) -- ($(EB\convid\nin)+(0.3*5/3,0)$) -- ($(EB\convid0)+(0.3*5/3,0)$) --cycle; 
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={-100+\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
            \draw[gray!80] (EB\convid\i) -- ($(EB\convid\i)+(0.3*5/3,0)$);
            \draw[gray!80] (DEB\convid\i) -- ($(EB\convid\i)+(0.3*5/3,0)$);
        \end{scope}
    }
    \draw[black] (EB\convid0) -- (EB\convid\nin) -- ($(EB\convid\nin)+(0.3*5/3,0)$) -- ($(EB\convid0)+(0.3*5/3,0)$) --cycle; 
    \draw[black] (DEB\convid0) -- (DEB\convid\nin) -- ($(EB\convid\nin)+(0.3*5/3,0)$) -- ($(EB\convid0)+(0.3*5/3,0)$) --cycle; 
}

\newcommand\fbconvv[4]{
    \def\nin{#1}
    \def\convid{#2}
    \def\xx{#3}
    \def\yy{#4}
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={100+\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
                \coordinate (EB\convid\i) at ($(\xx,\yy)+(0,0)$);
                \coordinate (DEB\convid\i) at ($(\xx,\yy)+(0.3*5/3,0.21*5/3)$);
              \gridd{EB\convid\i}{0.3*5/3}{0.21*5/3}
        \end{scope}
    }

    \draw[fill,gray!10,opacity=0.8] (EB\convid0) -- (EB\convid\nin) -- ($(EB\convid\nin)+(0.3*5/3,0)$) -- ($(EB\convid0)+(0.3*5/3,0)$) --cycle; 
    \draw[fill,gray!10,opacity=0.8] (DEB\convid0) -- (DEB\convid\nin) -- ($(EB\convid\nin)+(0.3*5/3,0)$) -- ($(EB\convid0)+(0.3*5/3,0)$) --cycle; 
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={100+\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
            \draw[gray!80] (EB\convid\i) -- ($(EB\convid\i)+(0.3*5/3,0)$);
            \draw[gray!80] (DEB\convid\i) -- ($(EB\convid\i)+(0.3*5/3,0)$);
        \end{scope}
    }
    \draw[black] (EB\convid0) -- (EB\convid\nin) -- ($(EB\convid\nin)+(0.3*5/3,0)$) -- ($(EB\convid0)+(0.3*5/3,0)$) --cycle; 
    \draw[black] (DEB\convid0) -- (DEB\convid\nin) -- ($(EB\convid\nin)+(0.3*5/3,0)$) -- ($(EB\convid0)+(0.3*5/3,0)$) --cycle; 
}

\newcommand\fbconvvv[4]{
    \def\nin{#1}
    \def\convid{#2}
    \def\xx{#3}
    \def\yy{#4}
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={100+\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
                \coordinate (EB\convid\i) at ($(\xx,\yy)+(0,0)$);
                \coordinate (DEB\convid\i) at ($(\xx,\yy)+(0.3*7/3,0.21*7/3)$);
              \griddd{EB\convid\i}{0.3*7/3}{0.21*7/3}
        \end{scope}
    }

    \draw[fill,gray!10,opacity=0.8] (EB\convid0) -- (EB\convid\nin) -- ($(EB\convid\nin)+(0.3*7/3,0)$) -- ($(EB\convid0)+(0.3*7/3,0)$) --cycle; 
    \draw[fill,gray!10,opacity=0.8] (DEB\convid0) -- (DEB\convid\nin) -- ($(EB\convid\nin)+(0.3*7/3,0)$) -- ($(EB\convid0)+(0.3*7/3,0)$) --cycle; 
    \foreach \i in {0,1,...,\nin} {
        \begin{scope}[  % Lower layer
            yshift={100+\channelwidth*\i},every node/.append style={
                 yslant=0,xslant=1,rotate=\rot},yslant=0,xslant=1,rotate=\rot
              ]              
            \draw[gray!80] (EB\convid\i) -- ($(EB\convid\i)+(0.3*7/3,0)$);
            \draw[gray!80] (DEB\convid\i) -- ($(EB\convid\i)+(0.3*7/3,0)$);
        \end{scope}
    }
    \draw[black] (EB\convid0) -- (EB\convid\nin) -- ($(EB\convid\nin)+(0.3*7/3,0)$) -- ($(EB\convid0)+(0.3*7/3,0)$) --cycle; 
    \draw[black] (DEB\convid0) -- (DEB\convid\nin) -- ($(EB\convid\nin)+(0.3*7/3,0)$) -- ($(EB\convid0)+(0.3*7/3,0)$) --cycle; 
}
\begin{figure*}[ht]
    \centering
\def\rot{0}
\def\dd{0.8}
\def\ggg{0.6}
\def\c{gray!10}
\def\d{green!20}
\def\channelwidth{6}
\def\fmw{1.0}
\def\fmh{0.7}
\resizebox{2.0\columnwidth}{!}{
\pgfdeclarelayer{fig}\pgfdeclarelayer{bg}
\pgfsetlayers{fig,bg}  
\begin{tikzpicture}[decoration={brace},font=\Large][scale=1,every node/.style={minimum size=1cm},on grid]
    \begin{pgfonlayer}{fig}
        \whitefm{4}{0}{-1.6}{0.0}{0}
        \bbconv{4}{0}{0.2}{0.15}
        \bbconv{4}{1}{1.0}{0.15}
        \bbconv{4}{2}{1.8}{0.15}
        \bbconv{4}{3}{2.6}{0.15}
        \gfm{4}{1}{4.5}{0.0}{green!20}
        \bbconv{4}{4}{6.3}{0.15}
        \bbconv{4}{5}{7.1}{0.15}
        \bbconv{4}{6}{7.9}{0.15}
        \gfm{3}{2}{9.8}{0.0}{red!20}
        \bbconv{3}{7}{11.6}{0.15}
        \bbconv{3}{8}{12.4}{0.15}
        \bbconv{3}{9}{13.2}{0.15}
        \bbconv{3}{10}{14.0}{0.15}
        \gfm{4}{3}{15.9}{0.0}{red!20}
        \bbconv{4}{11}{17.7}{0.15}
        \bbconv{4}{12}{18.5}{0.15}
        \bbconv{4}{13}{19.3}{0.15}
        \gfm{3}{4}{21.2}{0.0}{green!20}
        \bbconv{3}{14}{23.0}{0.15}
        \bbconv{3}{15}{23.8}{0.15}
        \bbconv{3}{16}{24.6}{0.15}
        \whitefm{3}{5}{26.5}{0.0}{0}
        \coordinate (id) at (3.9,0.5);
        \coordinate (id2) at (9.2,0.5);
        \coordinate (id3) at (20.6,0.5);
        \coordinate (act) at (15.35, 0.5);
        \coordinate (act2) at (25.95, 0.5);
        \draw[black, thick] (id) circle [radius=0.35];
        \draw[black, thick] ($(id) + (0.35*1.414/2,0.35*1.414/2)$) --($(id) + (-0.35*1.414/2,-0.35*1.414/2)$);
        \node[black] at ($(id)+(0,+0.75)$) {$\mathrm{id}$};
        \draw[black, thick] (id2) circle [radius=0.35];
        \draw[black, thick] ($(id2) + (0.35*1.414/2,0.35*1.414/2)$) --($(id2) + (-0.35*1.414/2,-0.35*1.414/2)$);
        \node[black] at ($(id2)+(0,+0.75)$) {$\mathrm{id}$};
        \draw[black, thick] (id3) circle [radius=0.35];
        \draw[black, thick] ($(id3) + (0.35*1.414/2,0.35*1.414/2)$) --($(id3) + (-0.35*1.414/2,-0.35*1.414/2)$);
        \node[black] at ($(id3)+(0,+0.75)$) {$\mathrm{id}$};

        \draw[blue!60!black!100, thick] (act) circle [radius=0.35];
        \draw[blue!60!black!100, thick] ($(act) + (-0.35,0)$) -- (act);
        \draw[blue!60!black!100, thick] ($(act) + (0.35*1.414/2,0.35*1.414/2)$) -- (act);
        \node[blue!60!black!100] at ($(act)+(0,-0.9)$) {ReLU};
        \node[blue!60!black!100] at ($(act)+(0,+0.7)$) {$\sigma_3$};
        % \draw[blue!60!black!100, thick] (act2) circle [radius=0.35];
        % \draw[blue!60!black!100, thick] ($(act2) + (-0.35,0)$) -- (act2);
        % \draw[blue!60!black!100, thick] ($(act2) + (0.35*1.414/2,0.35*1.414/2)$) -- (act2);
        % \node[blue!60!black!100] at ($(act2)+(0,-0.9)$) {ReLU};
        % \node[blue!60!black!100] at ($(act2)+(0,+0.7)$) {$\sigma_5$};
        \draw[black, thick] (act2) circle [radius=0.35];
        \draw[black, thick] ($(act2) + (0.35*1.414/2,0.35*1.414/2)$) --($(act2) + (-0.35*1.414/2,-0.35*1.414/2)$);
        %\node[blue!60!black!100] at ($(act2)+(0,-0.9)$) {ReLU};
        \node[black] at ($(act2)+(0,+0.75)$) {$\mathrm{id}$};
            \node[black!100] at ($(A03)+(1.1,1.45)$) {$X^{(0)}$};
    \node[black!100] at ($(A13)+(1.1,1.45)$) {$X^{(1)}$};
    \node[black!100] at ($(A22)+(1.1,1.7)$) {$X^{(2)}$};
    \node[black!100] at ($(A33)+(1.1,1.45)$) {$X^{(3)}$};
    \node[black!100] at ($(A43)+(1.1,1.45)$) {$X^{(4)}$};
    \node[black!100] at ($(A52)+(1.1,1.7)$) {$X^{(5)}$};
    
    \end{pgfonlayer}

\begin{pgfonlayer}{fig}
    \whitefm{4}{0}{0}{0.0}{-100}
    \bconvv{4}{1}{2.3}{0.0}
    \bconvv{4}{2}{3.9}{0.0}
    \bconvv{4}{3}{5.5}{0.0}
    \bfm{3}{1}{8.7}{0.0}{red!20}
    \bconv{3}{4}{10.6}{0.15}
    \bconv{3}{5}{11.6}{0.15}
    \bconv{3}{6}{12.6}{0.15}
    \bconv{3}{7}{13.6}{0.15}
    \bfm{4}{2}{15.9}{0.0}{red!20}
    \bconvv{4}{8}{18.2}{0.0}
    \bconvv{4}{9}{19.8}{0.0}
    \bconvv{4}{10}{21.4}{0.0}
    \whitefm{3}{3}{24.6}{0.0}{-100}
        \coordinate (act) at (15.28, -3.02);
        \coordinate (act2) at (23.7, -3.02);
        \coordinate (id) at (7.8,-3.02);
        \draw[black, thick] (id) circle [radius=0.35];
        \draw[black, thick] ($(id) + (0.35*1.414/2,0.35*1.414/2)$) --($(id) + (-0.35*1.414/2,-0.35*1.414/2)$);
        \node[black] at ($(id)+(0,+0.75)$) {$\mathrm{id}$};
        
        \draw[blue!60!black!100, thick] (act) circle [radius=0.35];
        \draw[blue!60!black!100, thick] ($(act) + (-0.35,0)$) -- (act);
        \draw[blue!60!black!100, thick] ($(act) + (0.35*1.414/2,0.35*1.414/2)$) -- (act);
        \node[blue!60!black!100] at ($(act)+(0,-0.9)$) {ReLU};
        \node[blue!60!black!100] at ($(act)+(0,+0.7)$) {$\sigma_3$};
        
        %\draw[blue!60!black!100, thick] (act2) circle [radius=0.35];
        %\draw[blue!60!black!100, thick] ($(act2) + (-0.35,0)$) -- (act2);
        %\draw[blue!60!black!100, thick] ($(act2) + (0.35*1.414/2,0.35*1.414/2)$) -- (act2);
        \draw[black, thick] (act2) circle [radius=0.35];
        \draw[black, thick] ($(act2) + (0.35*1.414/2,0.35*1.414/2)$) --($(act2) + (-0.35*1.414/2,-0.35*1.414/2)$);
        %\node[blue!60!black!100] at ($(act2)+(0,-0.9)$) {ReLU};
        \node[black] at ($(act2)+(0,+0.75)$) {$\mathrm{id}$};
    %\node at ($(B24)+(0.1,0.9)$) {$\theta_1\in\mathbb{R}^{C_1\times C_2\times K \times K}$};
    \node at ($(B24)+(0.3,1.)$) {$\theta_1\in\mathbb{R}^{4\times 4\times K\times K}$};
    %\node at ($(B54)+(0.9,0.9)$) {$\theta_2\in\mathbb{R}^{C_2\times C_3\times K \times K}$};
    \node at ($(B54)+(1.1,1.)$) {$\theta_2\in\mathbb{R}^{4\times 3\times K\times K}$};
    %\node at ($(B93)+(0.1,0.9)$) {$\theta_3\in\mathbb{R}^{C_3\times C_4\times K \times K}$};
    \node at ($(B93)+(0.3,1.25)$) {$\theta_3\in\mathbb{R}^{3\times 4\times K \times K}$};
    %\node at ($(B124)+(0.9,0.9)$) {$\theta_4\in\mathbb{R}^{C_4\times C_5\times K \times K}$};
    \node at ($(B124)+(1.1,1.)$) {$\theta_4\in\mathbb{R}^{4\times 3\times K \times K}$};
    %\node at ($(B153)+(0.9,0.9)$) {$\theta_5\in\mathbb{R}^{C_5\times C_6\times K \times K}$};
    \node at ($(B153)+(1.1,1.25)$) {$\theta_5\in\mathbb{R}^{3\times 3\times K \times K}$};

    % \node[red!60!black!100] at ($(A03)+(1.1,1.45)$) {$X^{(0)}$};
    % \node[black!100] at ($(A13)+(1.1,1.45)$) {$X^{(1)}$};
    % \node[red!60!black!100] at ($(A22)+(1.1,1.7)$) {$X^{(2)}$};
    % \node[red!60!black!100] at ($(A33)+(1.1,1.45)$) {$X^{(3)}$};
    % \node[black!100] at ($(A43)+(1.1,1.45)$) {$X^{(4)}$};
    % \node[red!60!black!100] at ($(A52)+(1.1,1.7)$) {$X^{(5)}$};
    

    % \coordinate (ABAB) at (17.75, 3.3);
    % \coordinate (ABABA) at (14.05, 3.3);
    % \node[blue!80] at (ABAB) {$\supset~ A=\{0,3,5\}$};
    % \node[red!80!black!100] at (ABABA) {$S=\{0,2,3,5\}$};

    
    \draw[thick,decorate,decoration={brace,amplitude=15pt,raise=4pt},line width=1pt] ($(B60)+(0.5,-0.2)$)--($(B00)+(0.0,-0.2)$) ;
    \node () at ($(B60)!0.5!(B00) + (1.85,-1.65)$) {$\theta_2 \circledast \theta_1\in\mathbb{R}^{4\times 3\times(2K-1)\times(2K-1)}$};
    \draw[thick,decorate,decoration={brace,amplitude=15pt,raise=4pt,aspect=0.65},line width=1pt] ($(B100)+(0.5,-0.2)$)--($(B70)+(0.0,-0.2)$) ;
    \node () at ($(B100)!0.5!(B70) + (0,-1.65)$) {$\theta_3\in\mathbb{R}^{3\times 4\times K\times K}$};
    \draw[thick,decorate,decoration={brace,amplitude=15pt,raise=4pt,aspect=0.65},line width=1pt] ($(B160)+(0.5,-0.2)$)--($(B110)+(0.0,-0.2)$) ;
    \node () at ($(B160)!0.5!(B110) + (0.6,-1.65)$) {$\theta_5 \circledast \theta_4\in\mathbb{R}^{4\times 3\times(2K-1)\times(2K-1)}$};


    % \node[red!60!black!100] at ($(BA03)+(1.1,1.45)$) {$X^{(0)}$};
    \node[red!60!black!100] at ($(BA13)+(1.1,1.45)$) {$X^{(2)}$};
    \node[red!60!black!100] at ($(BA23)+(1.1,1.45)$) {$X^{(3)}$};
    % \node[red!60!black!100] at ($(BA33)+(1.1,1.45)$) {$X^{(5)}$};
    \node[black!100] at ($(A03)+(1.1,1.45)$) {$X^{(0)}$};
    % \node[black!100] at ($(BA13)+(1.1,1.45)$) {$X^{(2)}$};
    % \node[black!100] at ($(BA23)+(1.1,1.45)$) {$X^{(3)}$};
    \node[black!100] at ($(A33)+(1.1,1.45)$) {$X^{(5)}$};
    \end{pgfonlayer}


\begin{pgfonlayer}{fig}
    \whitefm{4}{0}{5.0}{0.0}{100}
     \fbconvvv{4}{1}{7.6}{0.0}
     \fbconvvv{4}{2}{9.4}{0.0}
     \fbconvvv{4}{3}{11.2}{0.0}
     \fbconvvv{4}{3}{13}{0.0}
    % \bconv{3}{4}{10.6}{0.15}
    % \bconv{3}{5}{11.6}{0.15}
    % \bconv{3}{6}{12.6}{0.15}
    % \bconv{3}{7}{13.6}{0.15}
    \ffm{4}{2}{15.9}{0.0}{red!20}
    \fbconvv{4}{8}{18.2}{0.0}
    \fbconvv{4}{9}{19.8}{0.0}
    \fbconvv{4}{10}{21.4}{0.0}
    \whitefm{3}{3}{24.6}{0.0}{100}
        \coordinate (act2) at (23.7, 4.02);
        \draw[black, thick] (act2) circle [radius=0.35];
        \draw[black, thick] ($(act2) + (0.35*1.414/2,0.35*1.414/2)$) --($(act2) + (-0.35*1.414/2,-0.35*1.414/2)$);
        \node[black] at ($(act2)+(0,+0.75)$) {$\mathrm{id}$};
                \coordinate (act) at (15.28, 4.02);
        \draw[blue!60!black!100, thick] (act) circle [radius=0.35];
        \draw[blue!60!black!100, thick] ($(act) + (-0.35,0)$) -- (act);
        \draw[blue!60!black!100, thick] ($(act) + (0.35*1.414/2,0.35*1.414/2)$) -- (act);
        \node[blue!60!black!100] at ($(act)+(0,-0.9)$) {ReLU};
        \node[blue!60!black!100] at ($(act)+(0,+0.7)$) {$\sigma_3$};
    \node[black!100] at ($(A03)+(1.1,1.45)$) {$X^{(0)}$};
    \node[red!60!black!100] at ($(BA23)+(1.1,1.45)$) {$X^{(3)}$};
    \node[black!100] at ($(A33)+(1.1,1.45)$) {$X^{(5)}$};

    \draw[thick,decorate,decoration={brace,amplitude=15pt,raise=4pt,aspect=0.72},line width=1pt] ($(B03)+(0,+1.8)$)--($(B103)+(0.5,+1.8)$) ;
    \draw[thick,decorate,decoration={brace,amplitude=15pt,raise=4pt,aspect=0.3},line width=1pt] ($(B113)+(0,1.8)$)--($(B163)+(0.5,1.8)$) ;
    
    \node[black!100,align=left] at (28,4.4) {\textcolor{red!60!black!100}{$S=\{3\}$}\\{\textcolor{blue!60!black!100}{$A=\{3\}$}}};
    \node[black!100,align=left] at (28,-2.6) {\textcolor{red!60!black!100}{$S=\{2,3\}$}\\{\textcolor{blue!60!black!100}{$A=\{3\}$}}};
    \node () at ($(B160)!0.5!(B110) + (0.6,5.4)$) {$\theta_5 \circledast \theta_4\in\mathbb{R}^{4\times 3\times(2K-1)\times(2K-1)}$};
    \node () at ($(B160)!0.5!(B110) + (-9,5.4)$) {$\theta_3 \circledast (\theta_2\circledast \theta_1)\in\mathbb{R}^{4\times 4\times(3K-2)\times(3K-2)}$};
    \end{pgfonlayer}
    
\end{tikzpicture}
}
\label{fig:conv}
%\end{figure}
\caption{Illustration of merging the network according to $A = \{3\}$ and $S=\{2, 3\}$. The network  $\sigma_5 \circ f_{\theta_5} \circ f_{\theta_4}\circ \sigma_3 \circ f_{\theta_3} \circ f_{\theta_2}\circ f_{\theta_1}$ (above) is merged into the network $\sigma_5 \circ f_{\theta_5 \circledast \theta_4} \circ \sigma_3 \circ f_{\theta_3} \circ f_{\theta_2 \circledast \theta_1}$ (below) to accelerate the inference. Gray cuboids indicate the weights of the convolutional layer and the red cuboids indicate the places that we do not merge across. Note that we do not perform merging across the index $2$ to attain the optimal inference time.}
\end{figure*}


==> prop/dp.tex <==
\begin{proposition}
$A[l,t]$,and $S[l,t]$ computed from the DP recurrence relations, \Cref{eq:dprecur} are the optimal sets $A$ and $S$ of \Cref{eq:opt4}, respectively.
\label{prop:dp}
\end{proposition}
\begin{proof}
See supplementary material A for the detail.
\end{proof}

==> prop/lemma.tex <==
\begin{lemma}
\label{lemma:impa}
For given $A \subseteq [l-1]$, $A' = A\cup \{k\}$ and $k$ is the maximum element in $A'$. Then, 
\begin{align*}
I(A',0,l) &= I(A, 0, k) + I(k,l)
\end{align*}
\end{lemma}

\begin{proof}
Let $A'= \{a_1,\ldots,a_n\}$ where $a_1<\cdots<a_n=k$. 
Then, by the definition of $I(\cdot,\cdot,\cdot)$,
\begin{align*}
    I(A',0,l) &= \left(\sum_{j=1}^{n} I(a_{j-1},a_{j}) \right)+ I(a_n,l)\\
              &= \left(\sum_{j=1}^{n-1} I(a_{j-1},a_{j}) \right)+ I(a_{n-1},a_n) + I(a_n,l)\\
              &= \left(\sum_{j=1}^{n-1} I(a_{j-1},a_{j}) \right)+ I(a_{n-1},k) + I(k,l)\\
              &=I(A,0,k) + I(k,l)
\end{align*}
\end{proof}

\begin{lemma}
\label{lemma:times}
For given $S \subseteq [l-1]$, $S = S_{<k} \cup \{k\} \cup S_{>k}$ where $S_{<k} = \{s\in S\mid s< k\}$ and $S_{>k} = \{s\in S\mid s> k\}$. Then,
\begin{align*}
T(S,0,l) = T(S_{<k}, 0, k) + T(S_{>k},k,l)
\end{align*}
\end{lemma}

\begin{proof}
Let $S = \{s_1,\ldots,s_n\}$ where $s_1<\cdots<s_n$ and $s_m=k$.
Then, by the definition of $T(\cdot,\cdot,\cdot)$,
\begin{align*}
    T(S,0,l) &= 
    T(0,s_1)+\left(\sum_{i=2}^{n} T(s_{i-1},s_{i}) \right)+ T(s_n,l)\\
    &=  T(0,s_1)+\left(\sum_{i=2}^{m-1} T(s_{i-1},s_{i}) \right)+ T(s_{m-1},s_m) 
     + T(s_m, s_{m+1}) + \left(\sum_{i=m+1}^{n} T(s_{i-1},s_i) \right)+ T(s_n,l)\\
&= T(0,s_1)+\left(\sum_{i=2}^{m-1} T(s_{i-1},s_{i}) \right)+ T(s_{m-1},k) 
     + T(k, s_{m+1})+ \left(\sum_{i=m+2}^{n} T(s_{i-1},s_i) \right)+ T(s_n,l)\\
&=T(\{s_1,\ldots,s_{m-1}\},0,k) + T(\{s_{m+1},\ldots,s_n\},k,l)\\
&=T(S_{<k}, 0, k) + T(S_{>k},k,l)
\end{align*}
\end{proof}

==> tab/blks.tex <==

\begin{table}[t]
\caption{$\mathcal{B}$ denotes the set of positions that do not have activation in the original network. The following table enumerates the types of $I[l, k, a, j]$ that we take into account when we solve \Cref{alg:extDP}. Each cell has checkmark if the position belongs to $\mathcal{B}$ and is empty otherwise.}
\label{tab:blks}
\vspace{0.5em}
\centering

\begin{adjustbox}{max width=1.0\columnwidth}
\begin{tabular}{cccc}
\toprule
                        $l \in \mathcal{B}$ & $k \in \mathcal{B}$ & $a$
                            & $b$  \\
 \cmidrule(r){1-2}\cmidrule(r){3-4}
    & & 1 & 1 \\
 \cmidrule(r){1-2}\cmidrule(r){3-4}
    \cmark & & 1 & 1  \\
    \cmark & & 0 & 1  \\
 \cmidrule(r){1-2}\cmidrule(r){3-4}
     & \cmark & 1 & 1 \\
     & \cmark  & 1 & 0 \\
 \cmidrule(r){1-2}\cmidrule(r){3-4}
    \cmark & \cmark & 1  & 1  \\
    \cmark & \cmark & 0 & 1  \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}



==> tab/mbv2_1.0_in100.tex <==
\begin{table*}[t]
\caption{Accuracy and latency of compressed architectures applied to MobileNetV2-1.0 on ImageNet-100 dataset. The latency of the compressed network architecture is measured on \textit{TITAN Xp}, \textit{RTX 2080 Ti}, \textit{RTX 3090}, and  \textit{Tesla V100}.}
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=2.0\columnwidth}
\begin{tabular}{lcccccc}
\toprule
                            & 
                            & \multicolumn{4}{c}{TensorRT Latency (ms)} 
                            & \footnotesize{\textit{w/o} \normalsize{TensorRT (ms)}}\\
                            Network & Acc (\%) & \emph{TITAN Xp} & \emph{RTX 2080 Ti} & \emph{RTX 3090} 
                            & \emph{Tesla V100} 
                            & \emph{RTX 2080 Ti} \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MobileNetV2-1.0  & 87.58 & 27.58 & 19.55 & 14.38 & 17.17  & 40.68 \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-DS-A  &  85.60  & 20.14 & 15.01 & 10.51 & 13.38 &  27.71  \\
    % Ours& \textbf{86.22} & 20.26 & \textbf{14.85} & 11.08 & & &  \\
% \midrule
    MBV2-DS-B & 85.16 & 18.73 & 12.59 & 9.53 & 11.57 & 23.09  \\
    Ours      & \textbf{85.98} & \textbf{17.71} & \textbf{12.49} & \textbf{9.35} & 11.58 & \textbf{22.46}  \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-DS-C & 84.30 & 15.96 & 11.39 & 8.51 & 10.36 & 20.91  \\
    % Ours      & \textbf{84.72} & \textbf{15.30} & \textbf{11.20} & \textbf{8.43} & 10.58 & \textbf{20.41}\\
    Ours      & \textbf{84.36} & \textbf{15.32} & \textbf{10.50} & \textbf{7.88} & \textbf{10.14} & \textbf{18.39}\\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-DS-D & 83.18 & 14.68 & 10.65 & 7.89 & 10.00 & 18.91  \\
    Ours      & \textbf{84.00} & \textbf{13.71} & \textbf{9.92} & \textbf{7.43} & \textbf{9.87} &  \textbf{17.74}\\
\bottomrule
\end{tabular}
\end{adjustbox}
 \label{tab:in100-mbv2-1.0}
\end{table*}




					


















 
 






==> tab/mbv2_1.0_in100_rpr.tex <==

\begin{table}[t]
\caption{Accuracy and latency of compressed architectures applied to MobileNetV2-1.0 on ImageNet-100 dataset. 
Both compression methods use the latency information of  \textit{RTX 2080 Ti} and the latency is measured on the same \textit{RTX 2080 Ti}.}
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=1.0\columnwidth}
\begin{tabular}{lcccc}
\toprule
                            && \normalsize{TensorRT}
                            & \footnotesize{\textit{w/o}} \normalsize{TensorRT 
 }\\
                        Network     & Acc (\%)& Lat. (ms) & Lat. (ms)\\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    MBV2-1.0  & 87.58 & 19.55 & 40.68  \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-AR-1.0 & 85.46 & 13.32 & 24.48 \\
    Ours& \textbf{85.98}  & \textbf{12.49} & \textbf{22.46} \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-BR-1.0 & 83.92 & 11.86 & 20.96 \\
    Ours      & \textbf{84.36} & \textbf{10.50} & \textbf{18.39} \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-CR-1.0 & 83.24 & 10.82 & 17.95 \\
    Ours      & \textbf{84.00} & \textbf{9.92} & \textbf{17.74} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:rpr-in100-mbv2-1.0}
\end{table}




		
		


==> tab/mbv2_1.4_in100.tex <==
\begin{table*}[t]
\caption{Accuracy and latency of compressed architectures applied to MobileNetV2-1.4 on ImageNet-100 dataset. The latency of the compressed network architecture is measured on \textit{TITAN Xp}, \textit{RTX 2080 Ti}, \textit{RTX 3090}, and  \textit{Tesla V100}.}
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=2.0\columnwidth}
\begin{tabular}{lcccccc}
\toprule
                            & & \multicolumn{4}{c}{TensorRT Latency (ms)}   
                            & \footnotesize{\textit{w/o}} \normalsize{TensorRT (ms)}\\Network
                            & Acc (\%) & \emph{TITAN Xp} & \emph{RTX 2080 Ti} & \emph{RTX 3090} 
                            & \emph{Tesla V100} 
                            & \emph{RTX 2080 Ti} \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MobileNetV2-1.4  & 88.88 & 42.66 & 30.47 & 22.01 & 26.19  & 61.83 \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-1.4-DS-A  &  85.58  & 27.40 & 19.92 & 14.51 & 17.95 & 35.28  \\
    MBV2-1.4-DS-B  &  84.98  & 25.67 & 19.52 & 14.15 & 17.77 & 31.79 \\
    Ours& \textbf{86.16} & \textbf{25.44} & \textbf{18.74} & \textbf{13.44} & 18.03 & \textbf{31.22} \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-1.4-DS-C & 84.00 & 23.99 & 17.76 & 12.93 & 16.21 & 29.87 \\
    Ours      & \textbf{85.04} & \textbf{23.32} & \textbf{16.79} & \textbf{11.95} & \textbf{15.58} & \textbf{27.92} \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-1.4-DS-D & 83.02 & 23.00 & 17.77 & 12.81 & 15.87 & 28.09  \\
    MBV2-1.4-DS-E & 81.80 & 21.17 & 15.93 & 11.64 & 14.59 & 26.14  \\
    Ours      & \textbf{84.50} & \textbf{19.78} & \textbf{14.94} & \textbf{10.20} & \textbf{13.86} & \textbf{23.26} \\
% \midrule
    % MBV2-1.4-DS-F & 79.42 & 14.88 & 12.97 & 8.80 & 11.94 & &  17.13 & 17.13 \\
    % Ours      & \textbf{83.04} & 17.59 & 12.66 & & & & \\
    % Ours      & \textbf{80.00} & 15.03 & \textbf{11.40} & \textbf{7.52} & \textbf{10.96} & & \multicolumn{2}{c}{\textbf{16.97}}\\
\bottomrule
\end{tabular}
\end{adjustbox}
 \label{tab:in100-mbv2-1.4}
\end{table*}





































==> tab/mbv2_1.4_in100_rpr.tex <==

\begin{table}[t]
\caption{Accuracy and latency of compressed architectures applied to MobileNetV2-1.4 on ImageNet-100 dataset. Both compression methods use the latency information of  \textit{RTX 2080 Ti} and the latency is measured on the same \textit{RTX 2080 Ti}.} 
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=1.0\columnwidth}
\begin{tabular}{lccc}
\toprule
                            && \normalsize{TensorRT}
                            & \footnotesize{\textit{w/o}} \normalsize{TensorRT }\\
                        Network     & Acc (\%)& Lat. (ms)
                            & Lat. (ms) \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    MBV2-1.4  & 88.88 & 30.47 & 61.83 \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-AR-1.4  & 85.88 & 20.78 & 36.50 \\
    DS-BR-1.4 & 85.02 & 18.85 & 31.89 \\
    Ours& \textbf{86.16}  & \textbf{18.74} & \textbf{31.22} \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-CR-1.4 & 84.86 & 17.44 & 28.14 \\
    Ours      & \textbf{85.04} & \textbf{16.79} & \textbf{27.92} \\
% \midrule
    % MBV2-1.4-DS-F & 79.42 & 14.88 & 12.97 & 8.80 & 11.94 & &  17.13 & 17.13 \\
    % Ours      & \textbf{83.04} & 17.59 & 12.66 & & & & \\
    % Ours      & \textbf{80.00} & 15.03 & \textbf{11.40} & \textbf{7.52} & \textbf{10.96} & & \multicolumn{2}{c}{\textbf{16.97}}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:rpr-in100-mbv2-1.4}
\end{table}









==> tab/mbv2_1.4_in_noaug.tex <==
\begin{table*}[t]
\centering
\begin{adjustbox}{max width=1.0\columnwidth}
\begin{tabular}{l|c|ccccc|cc}
\toprule
    \multirow{2}{*}{Network}& \multirow{2}{*}{Accuracy (\%)}
                            & \multicolumn{5}{c|}{TensorRT Latency (ms)}
                            & \multicolumn{2}{c}{Non-TensorRT (ms)}\\
                            & & \emph{TITAN Xp} & \emph{RTX 2080 Ti} & \emph{RTX 3090} 
                            & \emph{Tesla V100} & \emph{Tesla A100}
                            & \emph{Fused BN} & \emph{Naive BN} \\
\midrule
    MobileNetV2-1.4  & 75.30 & 42.88 &  30.58 & 22.12 & 26.34 & & 62.01 & 68.38 \\
\midrule
    % MetaPruning-1.0$\times$  &  73.20  &  &  & & & & \\
    MBV2-1.4-DS-A  &  73.85  & 27.30 & 20.01 & 14.57 & 18.22 & & 35.44 & 38.67\\
    Ours & \textbf{74.22} & \textbf{26.27} & \textbf{18.96} & \textbf{14.00} & \textbf{17.62} & & \multicolumn{2}{c}{\textbf{32.79}} \\
\midrule
    MBV2-1.4-DS-B  &  73.19  & 25.74 & 19.66 & 14.17 & 17.67 & & 32.02 & 33.72\\
    Ours& \textbf{73.56} & \textbf{23.81} & \textbf{17.30} & \textbf{12.64} & \textbf{16.21} & & \multicolumn{2}{c}{\textbf{30.20}}\\
\midrule
    MBV2-1.4-DS-C & 72.69 & 24.15 & 17.79 & 12.89 & 16.67 & & 30.07 & 32.52\\
    MBV2-1.4-DS-D & 72.69 & 22.97 & 17.76 & 12.88 & 16.36 & & 28.35 & 29.53\\
    Ours& \textbf{73.06} & \textbf{22.81} & \textbf{16.67} & \textbf{12.06} & \textbf{15.38} & & \multicolumn{2}{c}{\textbf{27.90}}\\
\midrule
    MBV2-1.4-DS-E & 71.96 & 21.39 & 16.02 & 11.75 & 14.91 & & 26.39 & 28.30\\
    Ours      & \textbf{72.05} & \textbf{20.88} & \textbf{15.29} & \textbf{11.21} & \textbf{14.72} & & \multicolumn{2}{c}{\textbf{26.10}}\\
% \midrule
    % MetaPruning-0.35$\times$  &  64.50  & &  & & & &  \\
    % MetaPruning-0.65$\times$  &  71.70  & &  & & & &  \\
    % MBV2-1.4-DS-F & 67.76 & 14.91 & 13.04 & 8.88 & 12.14 & & 17.19 & 17.19\\
    % Ours      & \textbf{68.80} & 16.05 & \textbf{11.87} & \textbf{8.60} & \textbf{11.78} & & \multicolumn{2}{c}{18.29} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{MobileNetV2-1.4 @ImageNet with $\alpha = 1.2$ and without augmentation}
\end{table*}
























==> tab/mbv2_in100.tex <==


\begin{table}[t]
\caption{Accuracy and latency of compressed architectures applied to MobileNetV2-1.0 and MobileNetV2-1.4 on ImageNet-100 dataset. The latency of the compressed network architecture is measured on \textit{TITAN Xp}, \textit{RTX 2080 Ti}, \textit{RTX 3090}, and  \textit{Tesla V100}.}
\begin{subtable}[t]{\columnwidth}
\caption{MobileNetV2-1.0}
\centering
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{lcccccc}
\toprule
                            & 
                            & \multicolumn{4}{c}{TensorRT Latency (ms)} 
                            & \footnotesize{\textit{w/o} \normalsize{TensorRT (ms)}}\\
                            Network & Acc (\%) & \emph{TITAN Xp} & \emph{RTX 2080 Ti} & \emph{RTX 3090} 
                            & \emph{Tesla V100} 
                            & \emph{RTX 2080 Ti} \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MobileNetV2-1.0  & 87.58 & 27.58 & 19.55 & 14.38 & 17.17  & 40.68 \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-DS-A  &  85.60  & 20.14 & 15.01 & 10.51 & 13.38 &  27.71  \\
    % Ours& \textbf{86.22} & 20.26 & \textbf{14.85} & 11.08 & & &  \\
% \midrule
    MBV2-DS-B & 85.16 & 18.73 & 12.59 & 9.53 & 11.57 & 23.09  \\
    Ours      & \textbf{85.98} & \textbf{17.71} & \textbf{12.49} & \textbf{9.35} & 11.58 & \textbf{22.46}  \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-DS-C & 84.30 & 15.96 & 11.39 & 8.51 & 10.36 & 20.91  \\
    % Ours      & \textbf{84.72} & \textbf{15.30} & \textbf{11.20} & \textbf{8.43} & 10.58 & \textbf{20.41}\\
    Ours      & \textbf{84.36} & \textbf{15.32} & \textbf{10.50} & \textbf{7.88} & \textbf{10.14} & \textbf{18.39}\\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-DS-D & 83.18 & 14.68 & 10.65 & 7.89 & 10.00 & 18.91  \\
    Ours      & \textbf{84.00} & \textbf{13.71} & \textbf{9.92} & \textbf{7.43} & \textbf{9.87} &  \textbf{17.74}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:in100-mbv2-1.0}
\end{subtable}
\\
\vspace{1em}
\\
\begin{subtable}[t]{\columnwidth}
\caption{MobileNetV2-1.4}
\centering
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{lcccccc}
\toprule
                            & & \multicolumn{4}{c}{TensorRT Latency (ms)}   
                            & \footnotesize{\textit{w/o}} \normalsize{TensorRT (ms)}\\Network
                            & Acc (\%) & \emph{TITAN Xp} & \emph{RTX 2080 Ti} & \emph{RTX 3090} 
                            & \emph{Tesla V100} 
                            & \emph{RTX 2080 Ti} \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MobileNetV2-1.4  & 88.88 & 42.66 & 30.47 & 22.01 & 26.19  & 61.83 \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-1.4-DS-A  &  85.58  & 27.40 & 19.92 & 14.51 & 17.95 & 35.28  \\
    MBV2-1.4-DS-B  &  84.98  & 25.67 & 19.52 & 14.15 & 17.77 & 31.79 \\
    Ours& \textbf{86.16} & \textbf{25.44} & \textbf{18.74} & \textbf{13.44} & 18.03 & \textbf{31.22} \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-1.4-DS-C & 84.00 & 23.99 & 17.76 & 12.93 & 16.21 & 29.87 \\
    Ours      & \textbf{85.04} & \textbf{23.32} & \textbf{16.79} & \textbf{11.95} & \textbf{15.58} & \textbf{27.92} \\
\cmidrule(r){1-2}\cmidrule(r){3-6} \cmidrule(r){7-7}
    MBV2-1.4-DS-D & 83.02 & 23.00 & 17.77 & 12.81 & 15.87 & 28.09  \\
    MBV2-1.4-DS-E & 81.80 & 21.17 & 15.93 & 11.64 & 14.59 & 26.14  \\
    Ours      & \textbf{84.50} & \textbf{19.78} & \textbf{14.94} & \textbf{10.20} & \textbf{13.86} & \textbf{23.26} \\
% \midrule
    % MBV2-1.4-DS-F & 79.42 & 14.88 & 12.97 & 8.80 & 11.94 & &  17.13 & 17.13 \\
    % Ours      & \textbf{83.04} & 17.59 & 12.66 & & & & \\
    % Ours      & \textbf{80.00} & 15.03 & \textbf{11.40} & \textbf{7.52} & \textbf{10.96} & & \multicolumn{2}{c}{\textbf{16.97}}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:in100-mbv2-1.4}
\end{subtable}
\end{table}

==> tab/mbv2_rpr_in100.tex <==

\begin{table}[t]
\caption{Accuracy and latency of compressed architectures applied to MobileNetV2-1.0 and MobileNetV2-1.4 on ImageNet-100 dataset. 
Both compression methods use the latency information of  \textit{RTX 2080 Ti} and the latency is measured on the same \textit{RTX 2080 Ti}.}
\begin{subtable}[t]{0.48\columnwidth}
\caption{MobileNetV2-1.0 }
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=1.0\columnwidth}
\begin{tabular}{lcccc}
\toprule
                            && \normalsize{TensorRT}
                            & \footnotesize{\textit{w/o}} \normalsize{TensorRT 
 }\\
                        Network     & Acc (\%)& Lat. (ms) & Lat. (ms)\\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    MBV2-1.0  & 87.58 & 19.55 & 40.68  \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-AR-1.0 & 85.46 & 13.32 & 24.48 \\
    Ours& \textbf{85.98}  & \textbf{12.49} & \textbf{22.46} \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-BR-1.0 & 83.92 & 11.86 & 20.96 \\
    Ours      & \textbf{84.36} & \textbf{10.50} & \textbf{18.39} \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-CR-1.0 & 83.24 & 10.82 & 17.95 \\
    Ours      & \textbf{84.00} & \textbf{9.92} & \textbf{17.74} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:rpr-in100-mbv2-1.0}
\end{subtable}
\begin{subtable}[t]{0.48\columnwidth}
\caption{MobileNetV2-1.4} 
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=1.0\columnwidth}
\begin{tabular}{lccc}
\toprule
                            && \normalsize{TensorRT}
                            & \footnotesize{\textit{w/o}} \normalsize{TensorRT }\\
                        Network     & Acc (\%)& Lat. (ms)
                            & Lat. (ms) \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    MBV2-1.4  & 88.88 & 30.47 & 61.83 \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-AR-1.4  & 85.88 & 20.78 & 36.50 \\
    DS-BR-1.4 & 85.02 & 18.85 & 31.89 \\
    Ours& \textbf{86.16}  & \textbf{18.74} & \textbf{31.22} \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-CR-1.4 & 84.86 & 17.44 & 28.14 \\
    Ours      & \textbf{85.04} & \textbf{16.79} & \textbf{27.92} \\
% \midrule
    % MBV2-1.4-DS-F & 79.42 & 14.88 & 12.97 & 8.80 & 11.94 & &  17.13 & 17.13 \\
    % Ours      & \textbf{83.04} & 17.59 & 12.66 & & & & \\
    % Ours      & \textbf{80.00} & 15.03 & \textbf{11.40} & \textbf{7.52} & \textbf{10.96} & & \multicolumn{2}{c}{\textbf{16.97}}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:rpr-in100-mbv2-1.4}
\end{subtable}
\end{table}

==> tab/mbv2_small_in100.tex <==

\begin{table}[t]
\caption{Accuracy and latency of compressed architectures applied to MobileNetV2-1.0 and MobileNetV2-1.4 on ImageNet-100 dataset. Compression methods use the latency information of \textit{RTX 2080 Ti} and the latency is measured on the same \textit{RTX 2080 Ti}.} 
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=1.0\columnwidth}
\begin{tabular}{lccc}
\toprule
                            && \normalsize{TensorRT}
                            & \footnotesize{\textit{w/o}} \normalsize{TensorRT }\\
                        Network     & Acc (\%)& Lat. (ms)
                            & Lat. (ms) \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
       MBV2-1.0  & 87.58 & 19.55 & 40.68  \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-A-1.0  & 85.60 & 15.01 &  27.71   \\
    DS-B-1.0  &  85.16  & 12.59 &  23.09  \\
    Ours& \textbf{85.98}  & \textbf{12.49} & \textbf{22.46} \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-C-1.0 & 84.30 & 11.39 &  20.91 \\
    Ours      & \textbf{84.36} & \textbf{10.50} & \textbf{18.39} \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-D-1.0 & 83.18 & 10.65 &  18.91 \\
    Ours      & \textbf{84.00} & \textbf{9.92} & \textbf{17.74} \\
% \midrule
    % MBV2-1.4-DS-F & 79.42 & 14.88 & 12.97 & 8.80 & 11.94 & &  17.13 & 17.13 \\
    % Ours      & \textbf{83.04} & 17.59 & 12.66 & & & & \\
    % Ours      & \textbf{80.00} & 15.03 & \textbf{11.40} & \textbf{7.52} & \textbf{10.96} & & \multicolumn{2}{c}{\textbf{16.97}}\\
\cmidrule[0.5pt]{1-4}
% \cmidrule(r){1-4}
     MBV2-1.4  & 88.88 & 30.47 & 61.83 \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-A-1.4  &  85.58  & 19.92 & 35.28 \\
    DS-B-1.4  &  84.98  & 19.52 & 31.79 \\
    Ours& \textbf{86.16}  & \textbf{18.74} & \textbf{31.22} \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-C-1.4 & 84.00 & 17.76 & 29.87 \\
    Ours      & \textbf{85.04} & \textbf{16.79} & \textbf{27.92} \\
 \cmidrule(r){1-2}\cmidrule(r){3-3} \cmidrule(r){4-4}
    DS-D-1.4 & 83.02 & 17.77 & 28.09 \\
    DS-E-1.4 & 81.80 & 15.93 & 26.14 \\
    Ours      & \textbf{84.50} & \textbf{14.94} & \textbf{23.26} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:small-in100-mbv2-1.4}
\end{table}





==> tab/rn56_cifar.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l|ccccc}
\toprule
    \multirow{2}{*}{Network}& Acc
                            & \emph{TITAN} & \emph{RTX} & \emph{RTX} &  Num of \\
                            & (\%) & \emph{Xp} & \emph{2080Ti} & \emph{3090} & Acts \\
\midrule
    ResNet-56  &  &            &   &  & 56 \\
\midrule
    FPGM  &    & & & & 56 \\
    Ours&  & &  & &  \\
\midrule
    FPGM  &    & & & & 56 \\
    Ours&  & &  & &  \\
\bottomrule
\end{tabular}
\caption{ResNet-56 @CIFAR-10}
\label{tab:cifar}
\end{table}
